On Scalable and Efficient Computation of Large Scale Optimal Transport

Optimal Transport (OT) naturally arises in many machine learning applications, yet the heavy computational burden limits its wide-spread uses. To address the scalability issue, we propose an implicit generative learning-based framework called SPOT (Scalable Push-forward of Optimal Transport). Specifically, we approximate the optimal transport plan by a pushforward of a reference distribution, and cast the optimal transport problem into a minimax problem. We then can solve OT problems efficiently using primal dual stochastic gradient-type algorithms. We also show that we can recover the density of the optimal transport plan using neural ordinary differential equations. Numerical experiments on both synthetic and real datasets illustrate that SPOT is robust and has favorable convergence behavior. SPOT also allows us to efficiently sample from the optimal transport plan, which benefits downstream applications such as domain adaptation.

==> Tech_Report copy/abstract.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

%\vspace{-0.1in}

\begin{abstract}
%Optimal Transport (OT) naturally arises in many machine learning applications, yet the heavy computational burden limits its wide-spread uses. To address the scalability issue, we propose an implicit generative learning-based framework called SPOT (Scalable Push-forward of Optimal Transport). Specifically, we cast the optimal transport problem into a minimax problem via infinite dimensional  Lagrangian multipliers. We then parameterize the optimal transport plan and Lagrangian multipliers with neural networks. By such a parameterization, we can solve OT problems efficiently using primal dual stochastic gradient-type algorithms. We also show that we can recover the density corresponding to the optimal transport plan using neural ODEs. Numerical experiments on both synthetic and real datasets illustrate that SPOT has favorable convergence behavior. SPOT also allows us to efficiently sample from the optimal transport plan, which benefits downstream applications such as domain adaptation.

Optimal Transport (OT) naturally arises in many machine learning applications, yet the heavy computational burden limits its wide-spread uses. To address the scalability issue, we propose an implicit generative learning-based framework called SPOT (Scalable Push-forward of Optimal Transport). Specifically, we approximate the optimal transport plan by a pushforward of a reference distribution, and cast the optimal transport problem into a minimax problem. We then can solve OT problems efficiently using primal dual stochastic gradient-type algorithms. We also show that we can recover the density of the optimal transport plan using neural ordinary differential equations. Numerical experiments on both synthetic and real datasets illustrate that SPOT is robust and has favorable convergence behavior. SPOT also allows us to efficiently sample from the optimal transport plan, which benefits downstream applications such as domain adaptation.

\end{abstract}

==> Tech_Report copy/background.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

%\vspace{-0.15in}
\section{Background}
\label{sec:background}
%\vspace{-0.05in}

We briefly review some background knowledge on optimal transport and implicit generative learning.

{\bf Optimal Transport}: The idea of optimal transport (OT) originally comes from \citet{monge1781memoire}, which proposes to solve the following problem,
\begin{align}\label{eq:monge}
T^* = \argmin_{T(X)\sim \nu} \mathbb{E}_{X\sim \mu} [c(X, T(X))] ,
\end{align}
where $T(\cdot)$ is a mapping from the space of $\mu$ to the space of $\nu$. The mapping $T^*$ is referred to as \textit{Monge map}, and \eqref{eq:monge} is referred to as Monge formulation of optimal transport. 

Monge formulation, however, is not necessarily feasible. For example, when $X$ is a constant random variable and $Y$ is not, there does not exist such a map $T$ satisfying $T(X)\sim \nu$. The Kantorovich formulation of our interest in  \eqref{eq:intro} is essentially a relaxation of \eqref{eq:monge} by replacing the deterministic mapping with the coupling between $\mu$ and $\nu$. Consequently, \textit{Kantorovich formulation} is guaranteed to be feasible and becomes the classical formulation of optimal transport in existing literature \citep{benamou2015iterative, chizat2015unbalanced, frogner2015learning,solomon2015convolutional, xie2018fast}.

%The optimal expectation $\mathcal{W}(\mu,\nu)$, i.e. the \textit{Wasserstein distance}, is proved to be a distance that has multiple nice properties \cite{arjovsky2017towards, villani2008optimal}, and achieves great success in numerous applications \cite{bonneel2011displacement, arjovsky2017wasserstein, kusner2015word,singh2018wasserstein} as a way to measure the distance between two distributions. The optimal transport plan $\gamma^*$ is widely used in in economy \cite{carlier2012optimal}, geophysical models \cite{gross2016recent}, image analysis \cite{rubner1998metric, haker2004optimal} and domain adaptation \cite{courty2017joint,damodaran2018deepjdot}.

%The Kantorovich's formulation is latter become the classical formulation of optimal transport. Based on the the type of supports of $\mu$ and $\nu$, optimal transport problems are divided in to three cases - discrete case, semi-discrete case, and continuous case \cite{genevay2016stochastic}. Many algorithms are proposed to solve the discrete case. As aforementioned, \citet{cuturi2013sinkhorn} proposed Sinkhorn algorithm for the discrete case for entropically regularized OT, which significantly improves the efficiency of computing OT, and therefore opens a new era of the field. Inspired by Sinkhorn algorithm, a series of new algorithms are proposed to accommodate the instability problem of Sinkhorn [][] or target more specific applications [][]. In addition, some algorithms are proposed to solve exact OT in discrete case \cite{xie2018fast, li2018semantic}. Problems of continuous case can be cast into discrete case by discretization, but in this way the algorithms scales poorly with respect to both the dimension and the number of the data.

%\citet{genevay2016stochastic} is the first to propose to compute OT in continuous case and semi-discrete case with stochastic optimization method. Later, \citet{seguy2017large} extend the formulation to mapping estimation. 
%\citet{arjovsky2017wasserstein} uses the dual formulation of OT with Euclidean cost function. 
%Furthermore, under Euclidean cost function, the solution of transport plan is not unique, and therefore, usually not sparse, which would cause difficulty in applying it to downstream tasks.
%Also as a stochastic-based method, \citet{yang2018scalable} seeks to solve a different setting, where the unbalanced optimal transport problem between two measures with different total mass is considered.

%However, methods to compute the optimal transport plan remains to be undeveloped. 
%Different from existing work, we will adopt pushforward-based method to train a generative model for $\gamma^*$.

%\vspace{-0.05in}
\textbf{Implicit Generative Learning}: For generative learning problems, direct estimation of a probability density function is not always convenient. For example, we may not have enough prior knowledge to specify an appropriate parametric form of the probability density function (pdf). Even when an appropriate parametric pdf is available, computing the maximum likelihood estimator (MLE) can be sometimes neither efficient nor scalable. To address these issues, we resort to implicit generative learning, which do not directly specify the density. Specifically, we consider that the observed variable $X$ is generated by transforming a latent random variable $Z$ (with some known distribution $\rho$) through some unknown mapping $G(\cdot)$, i.e., $X=G(Z)$. We then can train a generative model by estimating $G(\cdot)$ with a properly chosen loss function, which can be easier to compute than MLE. Existing literature usually refer to the distribution of $G(Z)$ as the \textbf{push-forward} of reference distribution $\rho$. Such an implicit generative learning approach also enjoys an additional benefit: We only need to choose $\rho$ that is convenient to sample, e.g., uniform or Gaussian distribution, and we then can generate new samples from our learned distribution directly through the estimated mapping $G$ very efficiently.


%Pushforward has long been used in generative models  For example, $Z$ can be a low dimensional Gaussian random variable, and $G(Z)$ maps the input to the space of images, such that the distribution of $G(Z)$ is the same as the given image dataset. In this way, the distribution of the dataset is obtained implicitly, and unlimited amount of new samples can be generated efficiently. 

For many applications, the target distribution can be quite complicated, in contrast to the distribution $\rho$ being simple. This actually requires the mapping $G$ to be flexible. Therefore, we choose to represent G using deep neural networks (DNNs), which are well known for its universal approximation property, i.e., DNNs with sufficiently many neurons and properly chosen activation functions can approximate any continuous functions over compact support up to an arbitrary error. Early empirical evidence, including variational auto-encoder (VAE, \citet{kingma2013auto}) and generative adversarial networks (GAN, \citet{goodfellow2014generative}) have shown great success of parameterizing $G$ with DNNs. They further motivate a series of variants, which adopt various DNN architectures to learn more complicated generative models \citep{radford2015unsupervised, chen2016infogan,zhao2016energy, dai2017calibrating, jiang2018computation}.

%Since $\rho$ is usually chosen to be simple but the target distribution can be complicated, the mapping $G$ between them usually needs to be complicated. Because deep neural networks (DNNs) can theoretically approximate any complex functions with enough parameters, in variantional auto-encoder (VAE)  \cite{kingma2013auto} and generative adversarial networks (GAN) \cite{goodfellow2014generative}, $G$ is parametrized as a DNN. Both of the methods are later proved to be a great success. Since then, a series of variants with more complicated and refined architecture is proposed to further improve the training stability or the visual quality of the generated samples \cite{ radford2015unsupervised, chen2016infogan,zhao2016energy, dai2017calibrating}(Jiang et al. 2019).


%Variantional auto-encoder (VAE) \cite{kingma2013auto} and Generative adversarial networks (GAN) \cite{goodfellow2014generative} are two of the milestones that uses push-forward in training generative models. They both parametrize the mapping $G(\cdot)$ as neural networks. 
%A \textit{discriminator} is trained to measure the distance between the distribution of $G(Z)$ and the distribution of interest. 
%Later, a series of variants is proposed to further improve the training stability or the visual quality of the generated samples \cite{ radford2015unsupervised, chen2016infogan,zhao2016energy, dai2017calibrating}(Jiang et al. 2019).

Although the above methods cannot directly estimate the density of the target distribution, for certain applications, we can actually recover the density of $G(Z)$. For example, generative flow methods such as NICE \citep{dinh2014nice}, Real NVP \citep{dinh2016density}, and Glow \citep{kingma2018glow}) impose sparsity constraints on weight matrices, and exploit the hierarchical nature of DNNs to compute the densities layer by layer. Specifically, NICE proposed in \citet{dinh2014nice} denotes the transitions of densities within a neural network as
\begin{align*}
Z \xrightarrow{f_0} h_1 \xrightarrow{f_1}  h_2 \cdots h_{m}\xrightarrow{f_m} G(Z),
\end{align*}
where $h_i$ represents the hidden units of the $i$-th layer and $f_i$ is the transition function. NICE suggest to restrict the Jacobian matrices of $f_i$'s to be triangular. Therefore, $f_i$'s are reversible and the transition of density in each layer can be easily computed. More recently, \citet{chen2018neural} propose a neural ordinary differential equation (neural ODE) approach to compute the transition from $Z$ to $G(Z)$. Specifically, they introduce a dynamical formulation and parameterizing the mapping $G$ using DNNs with recursive structures: They use an ODE to describe how the input $Z$ gradually evolves towards the output $G(Z)$ in continuous time,
\begin{align*}
dz/dt = \xi(z(t),t),
\end{align*}
where $z(t)$ denotes the continuous time interpolation of $Z$, and $\xi(\cdot, \cdot)$ denotes a feedforward-type DNN. Without loss of generality, we choose $z(0) = Z$ and $z(1) = G(Z)$. Then under certain regularity conditions, the mapping $G(\cdot)$ is guaranteed to be reversible, and the density of $G(Z)$ can be computed in $\mathcal{O}(d)$ time, where $d$ is the dimension of $Z$ \citep{grathwohl2018ffjord}.

%Usually, only samples are accessible from implicit generative models. With some special cases of parametrization, however, we can also easily recover the density of the distribution using change-of-variable technique.   One special case is generative flow, where some constraints on the neural network architecture is imposed, such that the weight matrices have sparse structure. Works of this kind include NICE \cite{dinh2014nice}, Real NVP \cite{dinh2016density}, and Glow \cite{kingma2018glow}. Recently, \citet{chen2018neural} propose another kind of parametrization with continuous dynamics instead of directly the mapping $G(\cdot)$. Starting from input $Z$, the dynamical formulation describes how $Z$ gradually evolves to output $G(Z)$ with respect to time. Specifically, they use an ordinary differential equation (ODE) to describe a time-varying variable $z(t)$ ,
%\begin{align*}
%\frac{dz}{dt} = h(z(t),t),
%\end{align*}
%and specify $h(\cdot, \cdot)$ by a neural network. The mapping from $Z$ to $G(Z)$ is described by the initialization and the termination of the continous dynamics, i.e. $z(0)=Z$, and $z(1)=G(Z)$, respectively.  With some continuity condition, the mapping $G(\cdot)$ is reversible, and the density of $G(Z)$ is computable in $\mathcal{O}(D)$ time if density of $Z$ is given, where $D=\dim(\mathcal{Z})$ \cite{grathwohl2018ffjord}.








==> Tech_Report copy/conclusion.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

\vspace{-0.15in}
\section{Conclusion}
\vspace{-0.1in}
We propose the SPOT (Scalable Pushforward of Optimal Transport) framework to efficiently solve optimal transport problems. Specifically, we approximate optimal transport plan as a generative model parameterized by a deep neural network, and cast the optimal transport problem into a minimax optimization problem. We then introduce how to recover the density of the transport plan. Numerical experiments illustrate that SPOT not only has favorable convergence behavior, but is also capable to efficiently generate authentic samples. We finally apply SPOT to domain adaptation problems and achieve state-of-the-art performances. 

==> Tech_Report copy/discussion.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

%\vspace{-0.15in}
\section{Discussion}\label{sec:discussion}
%\vspace{-0.05in}

Existing literature shows that several stochastic algorithms can efficiently compute the Wasserstein distance between two continuous distributions. These algorithms, however, only apply to the dual of the OT problem \eqref{eq:intro}, and cannot provide the optimal transport plan. For example, \citet{genevay2016stochastic} suggest to expand the dual variables in two reproducing kernel Hilbert spaces. They then apply the Stochastic Averaged Gradient (SAG) algorithm to compute the optimal objective value of OT with continuous marginal distributions or semi-discrete marginal distributions (i.e., one marginal distribution is continuous and the other is discrete). The follow-up work, \citet{seguy2017large}, parameterize the dual variables with neural networks and apply the Stochastic Gradient Descent (SGD) algorithm to eventually achieve a better convergence. These two methods can only provide the optimal transport plan and recover the joint density when the densities of the marginal distributions are known. This is prohibitive in most applications, since we only have access to the empirical data. Our framework actually allows us to efficiently compute the joint density from the transformation of the latent variable $Z$ as in Section \ref{section4}.

%\textbf{Extension to Unbalanced Marginal Measures:} Many OT problems consider unbalanced marginal measures (e.g., supply and demand does not match in the resource allocation problem). A line of research suggests to use refined discrepancy measures between measures with different total mass \citet{liero2018optimal, KL-divergence}. For example, \citet{liero2018optimal}, instead of imposing strict equality constraints on the marginal distributions in \eqref{eq:intro}, add penalty terms to the objective using Csizs\'{a}r $f$-divergence. Then \eqref{eq:intro} can be rewritten as
%\begin{align*}
%\min_{G \in \cG} \EE_{Z}[c(G_X(Z), &G_Y(Z))] \\
%&+  \eta\big(d_{w}(G_X, X) + d_{w}(G_Y, Y)\big).
%\end{align*}
%A line of research suggest to 
%One approach for scalably computing the Wasserstein distance is through a variant of the dual formulation. These dual formulations are modified so that the number of variables are lower, and therefore, easier to parametrize in a way that stochastic optimization methods can be applied.
%\citet{genevay2016stochastic} is the first to propose to compute OT in continuous case and semi-discrete case with stochastic optimization method. Later, \citet{seguy2017large} extend the formulation to mapping estimation. 
%They both optimize the dual formulation of entropically regularized optimal transport problem, whereas \citet{seguy2017large}'s parametrization and optimization has a much better convergence.
%Their methods can retrieve the transport plan only if both the densities and samples are available, which is hardly the case in practice. Furthermore, the retrieving process is inevitably suspicious to the accumulation of numerical error.
%\citet{arjovsky2017wasserstein} proposed a formulation for unregularized OT that is specific to using Euclidean distance as a cost function. This formulation has a simpler dual form with a single variable which can be parameterized as a neural network. Despite its good performance in generative tasks, it cannot retrieve the transport plan from the dual solution since the solution does not have the continuity provided by the entropy regularization. 
%Furthermore, under Euclidean cost function, the solution of transport plan is not unique, and therefore, usually not sparse, which would cause difficulty in applying it to downstream tasks.

%Also as a stochastic-based method, \citet{yang2018scalable} seeks to solve a very different setting, where the Monge problem between two measures with different total mass is considered.

 %\citet{genevay2016stochastic} and \citet{seguy2017large} propose to  with stochastic averaged gradient (SAG) or stochastic gradient descent (SGD), parametrized with reproducing kernel Hilbert space or neural network (NN), respectively.   
% 
%\textbf{Unbalanced Kantorovich Formulation}  
% 
%{\color{red}How to define samples from a measure?}
% 
%SPOT can also handle cases where the two input measure is unbalanced, i.e. two input measures have different total mass, as long as one can draw samples from the input measures. 
%As pointed out in \eqref{eq:multi-gan}, we can rewrite our objective function as 
% \begin{align*}
%\min_{G \in \cG} \EE_{Z}[c(G_X(Z), &G_Y(Z))] \\
%&+  \eta\big(d_{w}(G_X, X) + d_{w}(G_Y, Y)\big).
%\end{align*}
%If the measures of $X$ and $Y$ is not balanced, since we only use samples from it, the total masses are automatically rescaled to 1. In other words, our formulation handles naturally the unbalanced optimal transport problems that allow mass variation . 
% 
%\citet{liero2018optimal} also suggest that for unbalanced optimal transport problem, we can relax the equality constraints in the initial Kantorovich formulation \eqref{eq:intro} to a penalization on marginal deviation using a divergence. Further, \citet{chizat2016scaling} adopt KL divergence for the marginals, and propose a Sinkhorn based algorithm for the discrete case. Our formulation is in consistent with theirs [][], although our formulation is for continuous case, and has better scalability.  

%Thus, the proposed objective function \eqref{eq:finalobjective} is consistent with the relaxed Kantorovich formulation \citep{liero2018optimal, chizat2015unbalanced}, when the divergences of marginal distributions are chosen to be the Wasserstein distance. 

%{\color{red}----------------------------------------}

%Another special case is when $\dim(\mathcal{Z})=\dim(\mathcal{X})=\dim(\mathcal{Y})$, we can parametrize both $G_{\mathcal{X}}$ and $G_{\mathcal{Y}}$ to be reversible \cite{schirrmeister2018generative, kingma2018glow, chen2018neural}. Assuming measure $\mu$ and $\nu$ are both continuous, the Monge map of both directions exist and can be computed from 
%\[
%\hat{X}=G_{\mathcal{X}}(G_{\mathcal{Y}}^{-1}(Y)), \quad \hat{Y}=G_{\mathcal{Y}}(G_{\mathcal{X}}^{-1}(X)).
%\]

==> Tech_Report copy/experiment1.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

%\vspace{-0.15in}
\section{Experiments}
%\vspace{-0.05in}

We evaluate the SPOT framework on various tasks: Wasserstein distance approximation, density recovery, paired sample generation and domain adaptation. All experiments are implemented with PyTorch using one GTX1080Ti GPU and a Linux desktop computer with 32GB memory, and we adopt the Adam optimizer with configuration parameters 0.5 and 0.999 \citep{kingma2014adam}.
%For practical reason, we optimize $\cL/\eta$ instead of $\cL$. The learning rate reported below corresponds to objective function $\cL/\eta$. 

%\vspace{-0.15in}
\subsection{Wasserstein Distance (WD) Approximation}
\label{section51}
%\vspace{-0.05in}

%\yujia{Results acknowledged by \citet{seguy2017large} .

We first demonstrate that SPOT can accurately and efficiently approximate the Wasserstein distance. We take the Euclidean ground cost, i.e. $c(x, y) = \norm{x - y}$. Then $\EE_{G(Z) \sim \gamma^*}[c(G_X(Z),G_Y(Z))]$ essentially approximates the Wasserstein distance. We take the marginal distributions $\mu$ and $\nu$ as two Gaussian distributions in $\RR^2$ with the same identity covariance matrix. The means are $(-2.5, 0)^\top$ and $(2.5, 0)^\top$, respectively. We find the Wasserstein distance between $\mu$ and $\nu$ equal to 5 by evaluating its closed-form solution. We generate $n = 10^5$ samples from both distributions $\mu$ and $\nu$, respectively. Note that naively applying discretization-based algorithms by dividing the support according to samples requires at least 40 GB memory, which is beyond the memory capability.

We parameterize $G_X$, $G_Y$, $\lambda_X$, and $\lambda_Y$ with fully connected neural networks without sharing parameters. All the networks use the Leaky-ReLU activation \cite{maas2013rectifier}. $G_X$ and $G_Y$ have $2$ hidden layers. $\lambda_X$ and $\lambda_Y$ have $1$ hidden layer. The latent variable $Z$ follows the standard Gaussian distribution in $\RR^2$. We take the batch size equal to 100. 

%We first test the ability to compute Wasserstein distance of SPOT. Since exact methods such as simplex network cannot tackle large number of data, it is difficult to obtain the ground truth to compare with. Therefore we adopt two Gaussian distributions as $\mu$ and $\nu$, in which case $\mathcal{W}(\mu, \nu)$ has close form. We also use very large number of data, i.e. $n=10^5$, so that the Wasserstein distance between the empirical distributions $\mathcal{W}(\hat{\mu}, \hat{\nu})$ is approximately the same as $\mathcal{W}(\mu, \nu)$.

%Specifically, the input distributions $\mu$ and $\nu$ are 2 dimensional Gaussian distributions with mean $(-3,0)$ and $(3,0)$ respectively and identity as variance, and the ground cost $c(\cdot,\cdot)$ is Euclidean distance. Both methods adopt Adam optimizer and batch size 100. For dual method \cite{seguy2017large}, we adopt the code from the authors\footnote{GitHub repository: https://github.com/vivienseguy/Large-Scale-OT} with only different input samples and parameter setting. For SPOT, we parameterize $G(\cdot)$ and $f_{\mathcal{X}}$, $f_{\mathcal{X}}$ both to be fully connected neural network with 1 hidden layer with 128 hidden units and LeakyReLU activation function, and the latent dimension is 8. 

\textbf{WD vs. Number of Epochs.} We compare the algorithmic behavior of SPOT and Regularized Optimal Transport (ROT, \citet{seguy2017large}) with different regularization coefficients. For SPOT, we set the number of units in each hidden layer equal to 8 and $\eta = 10^4$. %Since their method is based on the dual formulation, we refer regularization coefficients as the dual variable \textit{dual} method. 
For ROT, we adopt the code from the authors\footnote{https://github.com/vivienseguy/Large-Scale-OT} with only different input samples, learning rates, and regularization coefficients.
%%%%%%%USE REGULARIZED OT to DENOTE seguy2017large

Figure \ref{fig:conv} shows the convergence behavior of SPOT and ROT for approximating the Wasserstein distance between $\mu$ and $\nu$ with different learning rates. 
%Each result (except the ground truth) is averaged over 10 different datasets, and plotted with $\pm$ pointwise standard deviation. 
We observe that SPOT converges to the true Wasserstein distance with only 0.6\%, 0.3\%, and 0.3\% relative errors corresponding to Learning Rates (LR) $10^{-3}$, $10^{-4}$, and $10^{-5}$, respectively. In contrast, ROT is very sensitive to its regularization coefficient. Thus, it requires extensive tuning to achieve a good performance.
\begin{figure}[h]
%\vspace{-0.1in}
\begin{subfigure}[b]{0.27\textwidth}
      \includegraphics[height=0.7\textwidth]{figures/conv/f1e-3.png}
      \caption{LR =$10^{-3}$}
\end{subfigure}
\begin{subfigure}[b]{0.27\textwidth}
      \includegraphics[height=0.7\textwidth]{figures/conv/f1e-4.png}
      \caption{LR =$10^{-4}$}
\end{subfigure}\hspace{-1.8mm}
\begin{subfigure}[b]{0.27\textwidth}
      \includegraphics[height=0.7\textwidth]{figures/conv/f1e-5.png}
      \caption{LR =$10^{-5}$}
\end{subfigure}
%\vspace{-0.15in}
    \caption{{\label{fig:conv} \it Comparison of convergence between SPOT and ROT. All the curves are averaged over 50 runs with different random seeds, and the shaded areas represent the standard deviation.}}
%\vspace{-0.05in}
\end{figure}

%\textbf{Marginal Voilation} 
%
%\begin{figure}[h]
%%%\vspace{-0.1in}
%\centering     %%% not \center
%\includegraphics[width=0.49\textwidth]{figures/density_est_gaussian.png}
%%%\vspace{-0.15in}
%\caption{\label{fig:hid} {\color{red}Trail figure. Checking size} From left to right: (1) Ground truth density; (2) Estimated density of input samples; (3) Estimated density of generated samples under $\eta=10^{5}$ and LR $10^{-3}$; (4) Estimated density of generated samples under $\eta=10^{4}$ and LR $10^{-3}$. }
%%%\vspace{-0.15in}
%\end{figure}
%\begin{table}[h!]
%%%\vspace{-0.1in}
%\caption{\label{tab:violation} violation}
%\centering
%\begin{tabular}{l|l|ll}
%	\hline
%	&&& \\[-1.1em]
%	LR &          & $\eta=10^{5}$ & $\eta=10^{4}$\\ \hline
%	&&& \\[-1.1em]
%	\multirow{2}{*}{$10^{-3}$} & $\cR_1$ &  $0.22\pm0.02$         &     $0.19 \pm 0.02$      \\
%	& $\cR_2$ &   $0.25 \pm 0.01$        &   $0.30 \pm 0.01$       \\\hline
%	\multicolumn{4}{c}{Empirical WD between $\mu$ and $\mu$: $0.09 \pm 0.01$}\\ \hline
%\end{tabular}
%%%\vspace{-0.2in}
%\end{table}
%On the other hand, the converged value of dual method \cite{seguy2017large} is largely affected by its regularization coefficient. 
%In ROT, smaller regularization coefficient means larger regularization power, or larger penalty for violating the constrain. Since the estimated Wasserstein distance should be maximized, larger penalty would constrain the objective function to be smaller. \fbox{\textcolor{red}{make sense?}}
%Therefore, smaller regularization coefficient would lead to smaller estimated Wasserstein distance. 

%In addition, we report the violations of the marginal distributions, which can be approximated by 
%\begin{align*}
%& \cR_1 =  \big\lvert \mathbb{E}_{Z\sim \rho} [\lambda_{X}(G_{X} (Z))] - \mathbb{E}_{X\sim \mu}[\lambda_{X}(X)] \big\rvert, \\
%& \cR_2 = \big\lvert \mathbb{E}_{Z\sim \omega} [\lambda_{Y}(G_{Y} (Z))] -\mathbb{E}_{Y\sim \nu}[\lambda_{Y}(Y)] \big\rvert.
%\end{align*}
%the converged value of $\mathbb{E}_{Z\sim \omega} [f_{\mathcal{X}}(G_{\mathcal{X}} (Z))] -\mathbb{E}_{X\sim \mu}[f_{\mathcal{X}}(X)]+ \mathbb{E}_{Z\sim \omega} [f_{\mathcal{Y}}(G_{\mathcal{Y}} (Z))] -\mathbb{E}_{Y\sim \nu}[f_{\mathcal{Y}}(Y)]$. {\color{red}need a notation for it} 
%In fact, with learning rates $10^{-3}$ and $10^{-5}$, the violation is on average of the order $10^{-6}$. 
%Table \ref{tab:violation} shows that the violation is indeed negligible.
%We then evaluate the estimated marginal distributions. Specifically, we randomly generate $3000$ samples from our learnt generator, and $3000$ samples from $\mu$ and $\nu$, respectively. We then compute their empirical Wasserstein distances as follows,
%\begin{align*}
%& \cR_1 =  \min_{\gamma_{ij}} \sum_{i, j} \gamma_{ij}\norm{G_X(Z_i)-X_j} , \\
%& \cR_2 =  \min_{\gamma_{ij}} \sum_{i, j} \gamma_{ij}\norm{G_Y(Z_i)-Y_j} ,
%\end{align*}
%where $\gamma_{ij}$'s are required to satisfy $\sum_i \gamma_{ij} = {1}/{3000}$ for all $j=1,..,3000$ and $\sum_j \gamma_{ij} = {1}/{3000}$ for all $i=1,...,3000$ for both distances. Both distances are computed using the linear programming solver \texttt{Gurobi}. Table \ref{tab:violation} reports the results averaged over 10 runs.
%
%Note that $3000$ samples are generally speaking not enough to approximate WD to a high precision. {\color{red}{Empirical WD between 2 identical Gaussian}}
%
%Since the Wasserstein distance between which is quantified by
%
%
% shows the violation.
%
%
%\begin{table}[h!]
%%%\vspace{-0.1in}
%\caption{\label{tab:violation} violation}
%%\scalebox{0.95}{
%%\begin{tabular}{l|l|ll}
%%\hline
%%&&& \\[-1.1em]
%%LR &          & $\eta=10^{5}$ & $\eta=10^{4}$\\ \hline
%%&&& \\[-1.1em]
%%\multirow{2}{*}{$10^{-3}$} & $\cR_1$ &  $(5.0\pm 3.8)\times 10^{-7}$         &     $(4.4\pm 0.8)\times 10^{-6}$      \\
%%                                  & $\cR_2$ &   $(5.0\pm 3.9)\times 10^{-7}$        &   $(3.6\pm 1.0)\times 10^{-6}$       \\\hline
%%&&& \\[-1.1em]
%%\multirow{2}{*}{$10^{-4}$} & $\cR_1$ &   $(7.6\pm 8.0)\times 10^{-7}$         &    $ (8.8\pm 7.0)\times 10^{-7} $     \\
%%                                  & $\cR_2$ &  $(3.7\pm 4.2)\times 10^{-7}$         &    $ (1.1\pm 1.2)\times 10^{-6}$      \\\hline
%%&&& \\[-1.1em]
%%\multirow{2}{*}{$10^{-5}$} & $\cR_1$ &   $(4.1\pm 1.8)\times 10^{-5}$         &    $ (2.9\pm 3.4)\times 10^{-5} $     \\
%%                                  & $\cR_2$ &   $(2.2\pm 1.9)\times 10^{-5}$         &    $ (2.3\pm 2.7)\times 10^{-5} $      \\ \hline
%%\end{tabular}}
%\centering
%\begin{tabular}{l|l|ll}
%	\hline
%	&&& \\[-1.1em]
%	LR &          & $\eta=10^{5}$ & $\eta=10^{4}$\\ \hline
%	&&& \\[-1.1em]
%	\multirow{2}{*}{$10^{-3}$} & $\cR_1$ &  $0.22\pm0.02$         &     $0.19 \pm 0.02$      \\
%	& $\cR_2$ &   $0.25 \pm 0.01$        &   $0.30 \pm 0.01$       \\\hline
%	&&& \\[-1.1em]
%	\multirow{2}{*}{$10^{-4}$} & $\cR_1$ &   $0.15 \pm 0.02$         &    $0.24 \pm 0.02$     \\
%	& $\cR_2$ &  $0.15 \pm 0.02$         &    $0.13 \pm 0.01$      \\\hline
%	&&& \\[-1.1em]
%	\multirow{2}{*}{$10^{-5}$} & $\cR_1$ &   $0.12 \pm 0.01$         &    $0.20 \pm 0.01 $     \\
%	& $\cR_2$ &   $0.23 \pm 0.02$         &    $0.24 \pm 0.01$      \\ \hline
%	\multicolumn{4}{c}{Empirical WD between $\mu$ and $\mu$: $0.09 \pm 0.01$}\\ \hline
%\end{tabular}
%%%\vspace{-0.2in}
%\end{table}
%
%%\begin{figure}[htb!]
%%%%\vspace{-0.05in}
%%\centering
%%\includegraphics[width=0.49\textwidth]{figures/conv.png}
%%%%\vspace{-0.15in}
%%\caption{\label{fig:conv} Comparison of convergence between dual method in \cite{seguy2017large} and SPOT. The ground truth $\mathcal{W}(\mu,\nu)$ is computed from the close form solution of Wasserstein distance between two Gaussian distributions $\mu$ and $\nu$, while the other plots are the estimated Wasserstein distance between the empirical distributions $\hat{\mu}$ and $\hat{\nu}$. All the plotted curves correspond to 10 runs of the optimizer with different random seeds, and the shaded areas represent the standard deviation. %Note the curve of dual method learning rate 1e-3 and reg 0.5 has a very large variance, so we think it is not a good setting.
%%}
%%%%\vspace{-0.1in}
%%\end{figure}
%
%
%
%
%%\begin{figure}
%%\centering     %%% not \center
%%\subfigure{\caption{\label{fig:a} LR}\includegraphics[width=0.15\textwidth]{figures/conv/f1e-3.png}}
%%\subfigure{\label{fig:b}\includegraphics[width=0.15\textwidth]{figures/conv/f1e-4.png}}
%%\subfigure{\label{fig:c}\includegraphics[width=0.15\textwidth]{figures/conv/f1e-4.png}}
%%\caption{{\color{red}Figures (c) need change. }}
%%\end{figure}
%
%
%
%%\begin{figure}
%%\centering     %%% not \center
%%\subfigure{\label{fig:a}\includegraphics[width=0.4\textwidth]{figures/wd_nsamples.png}}
%%\subfigure{\label{fig:b}\includegraphics[width=0.4\textwidth]{figures/wd_nhiddim.png}}
%%\caption{{\color{red}Figures need change. Current 10 runs, 1e5 samples. Will change to 50 runs, 1e3 or 1e4 samples.}}
%%\end{figure}
%%
%%
%%\textbf{WD vs. number of samples} 
%%We then test on the sample efficiency of SPOT, i.e.  we test the accuracy of the estimated WD given a specific sample size. Here, we use learning rate $10^{-3}$, $1/\eta=10^{-4}$, and 8 units in each hidden layer. 
%%
%%\vspace{-0.05in}
\begin{wrapfigure}{R}{0.5\textwidth}
  \begin{center}
  \vspace{-20pt}
    \includegraphics[width=0.48\textwidth]{figures/wd_nhiddim.png}
  \end{center}
  \vspace{-10pt}
  \caption{\label{fig:hid}  Box plots of relative errors of the estimated Wasserstein distance with respect to the number of hidden units per layer. The results are averaged over 50 independent runs. }
  \vspace{-10pt}
\end{wrapfigure}

\textbf{WD vs. Number of Hidden Units.} 
We then explore the adaptivity of SPOT by increasing the network size, while the input data are generated from some low dimensional distribution. Specifically, the number of hidden units per layer varies from $2$ to $2^{10}$. Recall that we parameterize $G$ with two 2-hidden-layer neural networks, and $\lambda_X$, $\lambda_Y$ with two 1-hidden-layer neural networks. Accordingly, the number of parameters in $G$ varies from $36$ to about $2\times10^6$, and that in $\lambda_X$ or $\lambda_Y$ varies from $12$ to about $2,000$.  The tuning parameter $\eta$ also varies corresponding to the number of hidden units in $\lambda_X$, $\lambda_Y$. We use $\eta=10^{5}$ for $2^1, 2^2$ and $2^3$ hidden units per layer, $\eta=2\times 10^{4}$ for $2^4, 2^5$ and $2^6$ hidden units per layer, $\eta=10^{4}$ for $2^7$ and $2^8$ hidden units per layer, $\eta=2\times 10^{3}$ for $2^9$, and $2^{10}$ hidden units per layer.

%\begin{figure}[htb!]
%\vspace{-0.15in}
%\centering     %%% not \center
%\includegraphics[width=0.35\textwidth]{figures/wd_nhiddim.png}
%\vspace{-0.2in}
%\caption{\label{fig:hid} \it Box plots of relative errors of the estimated Wasserstein distance with respect to the number of hidden units per layer. The results are averaged over 50 independent runs. }
%\vspace{-0.1in}
%\end{figure}

Figure \ref{fig:hid} shows the estimated WD with respect to the number of hidden units per layer. For large neural networks that have $2^9$ or $2^{10}$ hidden units per layer, i.e., $5.2\times 10^{5}$ or $2.0\times10^{6}$ parameters, the number of parameters is far larger than the number of samples. Therefore, the model is heavily overparameterized. As we can observe in Figure \ref{fig:hid}, the relative error however, does not increase as the number of parameters grows. This suggests that SPOT is quite robust with respect to the network size.






==> Tech_Report copy/experiment2.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex



%\vspace{-0.1in}
\subsection{Density Recovery}
%\vspace{-0.05in}

We demonstrate that SPOT can effectively recover the joint density with entropy regularization. We adopt the neural ODE approach as described in Section \ref{section4}. Denote $\phi(a,b)$ as the density of the Gaussian distribution $N(a, b)$. We take the marginal distributions $\mu$ and $\nu$ as (1) Gaussian distributions $\phi(0,1)$ and $\phi(2,0.5)$; (2) mixtures of Gaussian $\frac{1}{2}\phi(-1,0.5)+\frac{1}{2}\phi(1,0.5)$ and $\frac{1}{2}\phi(-2,0.5)+\frac{1}{2}\phi(2,0.5)$.
The ground cost is the Euclidean square function, i.e., $c(x, y) = \norm{x - y}^2$. We run the training algorithm for $6 \times 10^5$ iterations and in each iteration, we generate 500 samples from $\mu$ and $\nu$, respectively. We parameterize $\xi$ with a 3-hidden-layer fully-connected neural network with 64 hidden units per layer, and the latent dimension is 2.  We take $\eta=10^6$.
%Besides the ability to compute Wasserstein distance, we also test the ability to explicit compute the transportation plan of SPOT. As pointed out in section \ref{section4}, explicitly computing the value of optimal transport can be easily done when we parametrize $G$ using neural ordinary differential equation. x1

\begin{wrapfigure}{R}{0.55\textwidth}
  \begin{center}
  \vspace{-10pt}
    \includegraphics[width=0.53\textwidth]{figures/entropy_gauss22.png}
  \end{center}
%  \vspace{-15pt}
  \caption{\label{fig:node}  Visualization of the marginal distributions and the joint density of the optimal transport plan. }
%  \vspace{-10pt}
\end{wrapfigure}

Figure \ref{fig:node} shows the input marginal densities and heat maps of output joint densities. We can see that a larger regularization coefficient $\epsilon$ yields a smoother joint density for the optimal transport plan. Note that with continuous marginal distributions and the Euclidean square ground cost, the joint density of the unregularized optimal transport degenerates to a generalized impulse function (i.e., a generalized Dirac $\delta$ function that has nonzero value on a manifold instead of one atom, as shown in \citet{rachev1985monge, onural2006impulse}). Entropy regularization prevents such degeneracy by enforcing smoothness of the density. 


%The input marginals and the output joint distribution is visualized in figure \ref{fig:node}. The method can adopt much higher dimensional input. We only adopt low dimensional input for visualization purpose. Adam optimizer and batch size 500 is used. We run each test 20,000 iterations, which is more than enough for convergence. The implementation of neural ODE and the corresponding parameter setting largely borrows \citep{grathwohl2018ffjord}.
%\footnote{GitHub repository: https://github.com/rtqichen/ffjord.} 
%\begin{figure}[htb!]
%\vspace{-0.1in}
%\centering
%\includegraphics[width=0.45\textwidth]{figures/node.png}
%\vspace{-0.15in}
%\caption{\label{fig:node} Visualization of optimal transport plan and the corresponding distributions for input samples. The positive directions of the figures are rightward and downward.}
%\vspace{-0.12in}
%\end{figure}






==> Tech_Report copy/experiment3.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

%\vspace{-0.15in}
\subsection{Sample Generation}
%\vspace{-0.05in}
\label{sec:section53}

\begin{figure*}[t!]
\centering
\includegraphics[width=0.99\textwidth]{figures/generated_mnist.png}
%\vspace{-0.12in}
\caption{\label{fig:generated_mnist} \it Generated samples of SPOT and CoGAN on the MNIST-MNISTM task.}
%\vspace{-0.15in}
\end{figure*}



We show that SPOT can generate paired samples $(G_X(Z), G_Y(Z))$ from unpaired data $X$ and $Y$ that are sampled from marginal distributions $\mu$ and $\nu$, respectively.

%With unpaired datasets $\{X_i\}$ and $\{Y_j\}$ as inputs, SPOT can generate paired data $(X,Y)$. 
%As suggested by \citet{liu2016coupled}, the learned joint distribution is useful in domain adaptation and image transformation. In synthetic datasets, we show that the marginal distributions are well satisfied, and the pair relationship is indeed optimal. In real image datasets, we show that the generated images are of high quality, and because the samples are generated from optimal transport plan, the paired relationship is clearer than \citet{liu2016coupled}, where the paired relationship is achieved by sharing parameters. 
%\vspace{-0.05in}


\begin{wrapfigure}{r}{0.45\textwidth}
  \begin{center}
%  \vspace{-15pt}
    \includegraphics[width=0.43\textwidth]{figures/synthetic.png}
  \end{center}
%  \vspace{-10pt}
  \caption{\label{fig:synthetic}  Visualization of input samples and generated samples. The black lines represent the paired relation. }
%  \vspace{-10pt}
\end{wrapfigure}

\textbf{Synthetic Data.} 
%The goal of this test is to visualize the generated samples and how they are paired together. 
We take the squared Euclidean cost, i.e. $c(x, y) = \norm{x - y}^2$, and adopt the same implementation and sample size as in Section \ref{section51} with learning rate $10^{-3}$ and 32 hidden units per layer. 
Figure \ref{fig:synthetic} illustrates the input samples and the generated samples with two sets of different marginal distributions: The upper row corresponds to the same Gaussian distributions as in Section \ref{section51}. The lower row takes $X$ as Gaussian distribution with mean $(-2.5,0)^\top$ and covariance $0.5I$, $Y$ as $(\sin (Y_1)+{Y}_2, 2Y_1-3)^\top$, where $Y_1$ follows a uniform distribution on $[0,3]$, and $Y_2$ follows a Gaussian distribution $N(2, 0.1)$. 
%The input distributions are visualized in figure \ref{fig:synthetic}.
%a) two Gaussian distributions same as section \ref{section51}, and b) one Gaussian distribution with mean $[-2,0]$ and variance 0.5, and one distribution 
%\begin{figure}[htb!]
%\centering
%\includegraphics[width=0.4\textwidth]{figures/synthetic.png}
%\vspace{-0.15in}
%\caption{\label{fig:synthetic} \it Visualization of input samples and generated samples. 
%%The colormap is aligned with the magnitude of the second dimension for each distribution. 
%The black lines represent the paired relation.}
%%In each plot, both the green and orange colormaps are aligned with the second dimension of $\tilde{Y}$ (the orange one), and therefore the paired relationship of different regions are visualized.}
%\end{figure}


We observe that the generated samples and the input samples are approximately identically distributed. Additionally, the paired relationship is as expected -- the upper mass is transported to the upper region, and the lower mass is transported to the lower region. 
%\textcolor{red}{To conclude the generated samples and the input samples are approximately identically distributed, don't we need to do density estimation for the generated samples? How can we observe the converged value of XXX? Paired relationship as expected?}

%\vspace{-0.05in}
\textbf{Real Data.} 
We next show SPOT is able to generate high quality paired samples from two unpaired real datasets: MNIST \citep{lecun1998gradient} and MNISTM \citep{ganin2014unsupervised}. The handwritten digits in MNIST and MNISTM datasets have different backgrounds and foregrounds (see Figrue \ref{fig:generated_mnist}). The digits in paired images however, are expected to have similar contours. We leverage this prior knowledge\footnote{For OT problems, $c$ can be viewed as a way to add prior knowledge to the problem \citep{peyre2017computational}.} by adopting a semantic-aware cost function \citep{li2018semantic} to extract the edge of handwritten letters, i.e., we use the following cost function
\begin{align*}
c(x,y)= \textstyle\sum_{i = 1}^2 \sum_{j = 1}^3 \left\lVert |C_i * x_j| - |C_i * y_j|\right\rVert_\textrm{F},
\end{align*}
where $C_1$ and $C_2$ denote the Sobel filter \citep{sobel1990isotropic}, and $x_j$'s and $y_j$'s are the three channels of RGB images. The operator $*$ denotes the matrix convolution. We set
\begin{align*}
C_1 = \begin{bmatrix}
-1&0&1\\
-2&0&2\\
-1&0&1
\end{bmatrix} ~~\textrm{and}~~
C_2 = \begin{bmatrix}
1&2&1\\
0&0&0\\
-1&-2&-1
\end{bmatrix},
\end{align*}
with $C_1$ and $C_2$ defining two extraction directions.

%We implement SPOT by parameterizing $G$, $\lambda_X$, and $\lambda_Y$ following \cite{radford2015unsupervised}.
We now use separate neural networks to parameterize $G_X$ and $G_Y$ instead of taking $G_X$ and $G_Y$ as outputs of a common network. Note that $G_X$ and $G_Y$ does not share parameters. Specifically,
we use two 4-layer convolutional layers in each neural network for $G_X$ or $G_Y$, and two 5-layer convolutional neural networks for $\lambda_{X}$ and $\lambda_{Y}$. More detailed network settings are provided in Appendix~\ref{sec:cnn_structure}. The batch size is 32, and we train the framework with $2\times 10^5$ iterations until the generated samples become stable.

%We first compare the generated result of SPOT and CoGAN \cite{liu2016coupled} using MNIST \cite{lecun1998gradient} and MNISTM \cite{ganin2014unsupervised}. In \cite{liu2016coupled}, the paired relationship of different domains is achieved by sharing parameters in the generators. Therefore, it is not explicitly guided by the objective function that how data points should be paired together. In SPOT, however, the paired relationship is guided by ground cost $c(\cdot,\cdot)$. Function $c$ is the cost to transport per unit of mass from a location in one domain to another domain -- when the two data points should be paired together, the cost should be smaller than when they should not be paired together. Therefore, the function $c$ is a perfect way for us to add domain knowledge to the formulation. For MNIST-MNISTM dataset, we are aware that the contour of the digits of the paired images should be the same. Therefore, borrowing ideas from \cite{li2018semantic}, we adopt a semantic-aware cost function
%\[
%c(u,v)=\left\lVert |\textbf{C}*u| - |\textbf{C}*v|\right\rVert_\textrm{F}
%\]
%where $\textbf{C} = \{C_1, C_2\}$ is the Sobel filter \citep{sobel1990isotropic},
%\[
%C_1 = \begin{bmatrix}
%-1&0&1\\
%-2&0&2\\
%-1&0&1
%\end{bmatrix},
%\quad C_2 = \begin{bmatrix}
%1&2&1\\
%0&0&0\\
%-1&-2&-1
%\end{bmatrix}
%\]
%are the edge extractors in the two directions of an image. {\color{red} Since convolution operation is a kind of linear operation, the cost function $c$ is a distance. } Note that other than the contour of the digits, the images from the MNISTM dataset also have contour of the photo patches that fills the foreground and background (see figrue \ref{fig:generated_mnist}), which is too complicated to be taken in to cost function explicitly. So the cost function $c$ we use here is just an approximated guidance of the paired relationship.

%For SPOT, the parametrization of $G_{\mathcal{X}}$, $G_{\mathcal{Y}}$, $f_{\mathcal{X}}$, $f_{\mathcal{X}}$ and parameter setting largely borrows from \cite{radford2015unsupervised}. For CoGAN \cite{liu2016coupled}, our code is adapted from Here\footnote{GitHub Repositories: https://github.com/mingyuliutw/CoGAN and https://github.com/eriklindernoren/PyTorch-GAN/blob/master/implementations/cogan/cogan.py}. Both methods uses batch size 32, and runs until the generated samples approximately do not change.

Figure \ref{fig:generated_mnist} shows the generated samples of SPOT. We also reproduce the results of CoGAN with the code from the authors\footnote{https://github.com/mingyuliutw/CoGAN}. As can be seen, with approximately the same network size, SPOT yields paired images with better quality than CoGAN: The contours of the paired results of SPOT are nearly identical, while the results of CoGAN have no clear paired relation. Besides, the images corresponding to $G_Y(Z)$ in SPOT have colorful foreground and background, while in CoGAN there are only few colors. Recall that in SPOT, the paired relation is encouraged by ground cost $c$, and in CoGAN it is encouraged by sharing parameters. By leveraging prior knowledge in ground cost $c$, the paired relation is more accurately controlled without compromising the quality of the generated images. 


%The reason behind is that in SPOT, the ground cost function encourages such a paired relation.

%The reason behind is that SPOT not only encourages the paired relation by parameter sharing but also by the ground cost function $c$.
%SPOT yields paired samples, since the parameter sharing in the generator $G$ and the ground cost function $c$ both encourage such a correspondence. This paired relationship however, is hardly seen in CoGAN. The reason behind is that CoGAN can only encourage paired relation by parameter sharing. 

We further test our framework on more complex real datasets: Photo-Monet dataset \cite{zhu2017unpaired} and Edges-Shoes dataset \cite{isola2017image}. We adopt the Euclidean cost function for Photo-Monet dataset, and the semantic-aware cost function as in MNIST-MNISTM for Edges-Shoes dataset. Other implementations remain the same as the MNIST-MINSTM experiment. 

Figure \ref{fig:generated_real} demonstrates the generated samples of both datasets. We observe that the generated images have a desired paired relation: For each $Z$, $G_X(Z)$ and $G_Y(Z)$ gives a pair of corresponding scenery and shoe. The generated images are also of high quality, especially considering that Photo-Monet dataset is a pretty small but complex dataset with 6,288 photos and 1,073 paintings. 

%Since SPOT has a clear guidance of how to pair images, the generated images has good paired relationship. On the other hand, the generated images of CoGAN do not show the paired relationship we want.
%For image generation, MNIST is a rather toy example. We further test SPOT's ability to generate paired images when images are larger and more complicated. Figure \ref{fig:generated_real} shows the generated images of Photo-Monet dataset \cite{zhu2017unpaired} and Edges-Shoes dataset \cite{isola2017image}. For Photo-Monet dataset, we use Euclidean cost function. For Sketches-Shoes dataset, we use the semantic-aware cost function same as MNIST-MNISTM. The implementation is the same as MNIST-MNSITM test. The generated samples in figure \ref{fig:generated_real} demonstrated that SPOT is capable to achieve optimal joint distribution as well as satisfy the marginal constrains for high dimensional data.

\begin{figure}[t!]
\centering
\includegraphics[width=0.98\textwidth]{figures/generate_complex1.png}
%\vspace{-0.15in}
\caption{\label{fig:generated_real} \it Generated samples of SPOT on Photos-Monet and Sketches-Shoes datasets.}
%\vspace{-0.15in}
\end{figure}

==> Tech_Report copy/experiment4.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

%\vspace{-0.15in}
\subsection{Domain Adaptation}\label{sec:DA}
%\vspace{-0.05in}


%Specifically, we jointly train the joint distribution and two classifiers, one for $X$ and one for $Y$. The joint distribution is trained using SPOT framework. We adopt a trainable ground cost $c(x,y) = \norm{D_{e,X}(x)-D_{e,Y}(y)}^2$, where $D_{e,X}$ and $D_{e,Y}$ are two trainable embedding networks that capture the high level features of $X$ and $Y$. This ground cost function encourages $X$ and $Y$ to be paired together if their embeddings have small Euclidean distance. We also train two linear classifiers, $D_{c,X}$ and $D_{c,Y}$, using the embeddings of $X$ and $Y$ as input. Accordingly, the classifiers of $X$, $Y$ can be also written as $D_X = D_{c,X} \circ D_{e,X}$ and $D_Y = D_{c,Y} \circ D_{e,Y}$, with $X$ and $Y$ as input. 
%The classifier $D_X$ is trained on input data $\{x_i, v_i\}$ in order to extract the label information. Since $(G_X(Z),G_Y(Z))$ is trained to follow the optimal transport plan, $G_X(Z)$, $G_Y(Z)$ should have the same label. Therefore, we also penalize the difference of $D_X(G_X(Z))$ and $D_Y(G_Y(Z))$.
%To sum up, the objective function can be written as $\cL + \eta_{\textrm{da}} \EE_{(X,V)}[\cL_c(D_X(X),V)] + \eta_{\textrm{da}}'  \EE_Z[\cL_c(D_Y(G_Y(Z)),\argmax_{k}[D_X(G_X(Z))]_k)]$, where $\cL$ is the objective function of OT problem in \eqref{eq:finalvariant}, $\cL_c$ is the cross entropy loss, $\eta_{da}, \eta'_{da}$ are the trade-off parameters, and $V$ is the random variable denoted for the label of $X$.
%We find such a coupling by adopting the SPOT framework to solve the OT problem between $\mu$ and $\nu$ with ground cost $c(x,y) = \norm{D_{e,X}(x)-D_{e,Y}(y)}^2$, where $D_{e,X}$ and $D_{e,Y}$ are two trainable embedding networks. This ground cost function encourages $X$ and $Y$ to be paired together if their embeddings have small Euclidean distance. We then build two classifiers based on the embedding networks as $D_X = D_{c,X} \circ D_{e,X}$ and $D_Y = D_{c,Y} \circ D_{e,Y}$, where $D_{c,X}, D_{c,Y}$ are linear classifiers. The choice of $D_{c,X}$ enables the embeddings of $X$ to have benign cluster structures, i.e., the data that has the same label belongs to the same clusters. Recall that the ground cost is defined as the distance between $D_{e, Y}(Y)$ and $D_{e, X}(X)$. Therefore, the embeddings of $Y$is encouraged to mimic that of $X$. Accordingly, the embeddings of $Y$ can inherit the structure of clusters in the embeddings of $X$, which largely benefits the training of $D_Y$.
%We train the SPOT and classifiers jointly by optimizing $\cL + \eta_{\textrm{da}} \cL_c(D_X(x),v) + \eta_{\textrm{da}}'  \cL_c(D_Y(y),D_X(x))$, where $\cL$ is the objective function of OT problem in \eqref{eq:finalvariant}, $\cL_c$ is the cross entropy loss, and $\eta_{da}, \eta'_{da}$ are the trade-off parameters.
% Here we choose $D_{c,X}, D_{c,Y}$ as linear classifiers to enforce $D_{e, X}(x)$ and $D_{e, Y}(y)$ to have benign cluster structures for an effective classification.
%To promote a better structure of clusters in $D_{e, X}(x)$ and $D_{e, Y}(y)$, we adopt $D_{c,X}, D_{c,Y}$ as linear classifiers.   This is because the ground cost function encourages the embedding of $Y$ to mimic that of $X$. Accordingly, $D_{e, Y}(y)$ can inherit the structure of clusters in $D_{e, X}(x)$, which largely benefits the training of classifiers for the target data $Y$. 
%In the training, the classifiers and SPOT are jointly trained by optimizing $\cL + \eta_{\textrm{da}} \cL_c(D_X(x),v) + \eta_{\textrm{da}}'  \cL_c(D_Y(y),D_X(x))$, where $\eta_{da}, \eta'_{da}$ are trade-off parameters and $\cL_c$ is the cross entropy loss.
%To enable the ground cost to assign smaller value to the paired data that should have the same label,  we use shared layers in the embedding networks and the classifiers,
%SPOT can be applied to domain adaptation since the optimal transport plan is essentially a coupling of $\mu$ and $\nu$. To make the transport plan similar to the wanted coupling, we adopt a trainable ground cost with discriminative power. Specifically, we define $c(x,y) = \norm{D_{e,X}(x)-D_{e,Y}(y)}^2$, where $D_{e,X}$ and $D_{e,Y}$ are two trainable embedding networks. 
%To enable the ground cost to assign comparably smaller value to the paired data that should have the same label,  we use shared layers in the embedding networks and the classifiers,
%i.e., we define two classifiers as $D_X = D_{c,X} \circ D_{e,X}$ and $D_Y = D_{c,Y} \circ D_{e,Y}$, where $D_{c,X}, D_{c,Y}$ are linear classifiers. 
%In the training, the classifiers and SPOT are jointly trained by optimizing $\cL + \eta_{\textrm{da}} \cL_c(D_X(x),v) + \eta_{\textrm{da}}'  \cL_c(D_Y(y),D_X(x))$, where $\eta_{da}, \eta'_{da}$ are trade-off parameters and $\cL_c$ is the cross entropy loss.
%For classification tasks, we parameterize the classifiers as $D_X = D_{c,X} \circ D_{e,X}$ and $D_Y = D_{c,Y} \circ D_{e,Y}$, where $D_{e,X}, D_{e,Y}$ are embedding networks and $D_{c,X}, D_{c,Y}$ are linear classifiers. We define the ground cost as: $c(x,y) = \norm{D_{e,X}(x)-D_{e,Y}(y)}^2$. We jointly train the classifier by adding an additional loss term $ \eta_{\textrm{da}} \cL_c(D_X(x),v) + \eta_{\textrm{da}}'  \cL_c(D_Y(y),D_X(x))$, where $\eta_{da}, \eta'_{da}$ are trade-off parameters and $\cL_c$ is the cross entropy loss.
%{\color{red}Maybe:We define the ground cost as: $c(x,y) = \norm{D_{e,X}(x)-D_{e,Y}(y)}^2+ \eta_{\textrm{da}}'  \cL_c(D_Y(y),D_X(x))$. We jointly train the classifier of source data by adding an additional loss term $ \eta_{\textrm{da}} \cL_c(D_X(x),v) $, where $\eta_{da}, \eta'_{da}$ are trade-off parameters and $\cL_c$ is the cross entropy loss.}
We choose $\eta_{\textrm{s}} = 10^3$ for all experiments. We set $\eta_{\textrm{da}}=0$ for the first $10^5$ iteration to wait the generators to be well trained. Then we set $\eta_{\textrm{da}}=10$ for the next $3\times 10^5$ iteration. We take totally $4\times 10^5$ iterations, and set the learning rate equal to $10^{-4}$ and batch size equal to $128$ for all experiments. 

We evaluate DASPOT with the MNIST, MNISTM, USPS \citep{hull1994database}, and SVHN \citep{netzer2011reading} datasets. We denote a domain adaptation task as Source Domain $\rightarrow$ Target Domain. 
%The model is trained with labeled training data from source domain and unlabeled training data from target domain. Then the model is tested with labeled testing data from target domain. 
For the tasks MNIST $\rightarrow$ USPS, USPS $\rightarrow$ MNIST and MNIST $\rightarrow$ MNISTM, we use three 4-layer networks for $D,\lambda_X$,and $\lambda_Y$, and two 5-layer networks for $G_X$ and $G_Y$. For the task SVHN $\rightarrow$ MNIST, we use three 5-layer downsampling ResNets \cite{he2016deep} for $D,\lambda_X,$ and $\lambda_Y$, and two 5-layer upsampling ResNets for $G_X$ and $G_Y$. More detailed implementations are provided in Appendices~\ref{sec:cnn_structure} and \ref{sec:resnet_structure}.



\begin{wraptable}{r}{0.6\linewidth}
%\vspace{-0.1in}
\caption{\it Domain Adaptation Experiments on multiple tasks.}
\label{tab:DAexp}
\scalebox{1.2}
{\footnotesize
\begin{tabular}{l|l|l|l|l}
		\hline
		Source		&  MNIST	&  USPS 	&  SVHN 	&  MNIST\\ 
		Target		&  USPS 	&  MNIST	&  MNIST	&  MNISTM\\ \hline
		%CoGAN 		&  $91.2\%$	&  $89.1\%$	&  $-$		&  $62.0\%$ \\ \hline
		%UNIT 		&  $96.0\%$	&  $93.6\%$	&  $90.5\%$	&  $-$ \\ \hline
		ROT 	&  $72.6\%$	&  $60.5\%$	&  $62.9\%$	&  $-$ \\ \hline
		StochJDOT 	&  $93.6\%$	&  $90.5\%$	&  $67.6\%$	&  $66.7\%$ \\ \hline
		DeepJDOT 	&  $95.7\%$	&  $96.4\%$	&  $\textbf{96.7\%}$	&  $92.4\%$ \\ \hline
		DASPOT 		&  $\textbf{97.5\%}$	&  $\textbf{96.5\%}$	&  $96.2\%$	&  $\textbf{94.9\%}$ \\ \hline
\end{tabular}}
%\vspace{-0.15in}
\end{wraptable} 

We compare the performance of DASPOT with other optimal transport based domain adaptation methods: ROT \citep{seguy2018large}, StochJDOT \citep{damodaran2018deepjdot} and DeepJDOT \citep{damodaran2018deepjdot}. As can be seen in Table \ref{tab:DAexp}, DASPOT achieves equal or better performances on all the tasks.

%
%\begin{table}[!htb]
%\vspace{-0.2in}
%\centering
%\caption{\it Domain Adaptation Experiments on multiple tasks.}
%\label{tab:DAexp}
%%\scalebox{0.95}
%{\footnotesize
%\begin{tabular}{l|l|l|l|l}
%		\hline
%		Source		&  MNIST	&  USPS 	&  SVHN 	&  MNIST\\ 
%		Target		&  USPS 	&  MNIST	&  MNIST	&  MNISTM\\ \hline
%		%CoGAN 		&  $91.2\%$	&  $89.1\%$	&  $-$		&  $62.0\%$ \\ \hline
%		%UNIT 		&  $96.0\%$	&  $93.6\%$	&  $90.5\%$	&  $-$ \\ \hline
%		ROT 	&  $72.6\%$	&  $60.5\%$	&  $62.9\%$	&  $-$ \\ \hline
%		StochJDOT 	&  $93.6\%$	&  $90.5\%$	&  $67.6\%$	&  $66.7\%$ \\ \hline
%		DeepJDOT 	&  $95.7\%$	&  $96.4\%$	&  $\textbf{96.7\%}$	&  $92.4\%$ \\ \hline
%		DASPOT 		&  $\textbf{97.5\%}$	&  $\textbf{96.5\%}$	&  $96.2\%$	&  $\textbf{94.9\%}$ \\ \hline
%\end{tabular}}
%\vspace{-0.22in}
%\end{table}

Moreover, we show that DeepJDOT is not as efficient as DASPOT. 
For example, in the MNIST $\rightarrow$ USPS task, DASPOT requires $169$s running time to achieve a $95\%$ accuracy, while DeepJDOT requires $518$s running time to achieve the same accuracy. The reason behind is that DeepJDOT needs to solve a series of optimal transport problems using Sinkhorn algorithm. The implementation of DeepJDOT is adapted from the authors' code\footnote{https://github.com/bbdamodaran/deepJDOT}.

%DASPOT is much more efficient, comparing to StochJDOT and DeepJDOT, where we need to solve a series of optimal transport problems using Sinkhorn algorithm. We compare the run time per iteration between SPOT and DeepJDOT on the task MNIST $\rightarrow$ MNISTM. Since DeepJDOT does not provide an official code for the task, to make a fair comparison, we implement DeepJDOT with PyTorch and POT package \cite{flamary2017pot}. With the same classifier architecture, SPOT takes $\bm{0.073 \pm 0.02}$s per iteration, while DeepJDOT takes $\bm{1.710 \pm 0.02}$s. 


==> Tech_Report copy/intro.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

%\vspace{-0.25in}
\section{Introduction}
%\vspace{-0.05in}

The Optimal Transport (OT) problem naturally arises in a variety of machine learning applications, where we need to handle data from multiple sources. One example is domain adaptation: We collect multiple datasets from different domains, and we need to learn a model from a source dataset, which can be further adapted to target datasets \citep{ganin2014unsupervised,courty2017optimal,damodaran2018deepjdot}. Another example is resource allocation: We want to assign a set of assets (one data source) to a set of receivers (another data source) so that an optimal economic benefit is achieved \citep{santambrogio2010models,galichon2017survey}. Recent literature has shown that both aforementioned applications can be formulated as optimal transport problems.

The optimal transport problem has a long history, and its earliest literature dates back to \citet{monge1781memoire}. Since then, it has attracted increasing attention and been widely studied in multiple communities such as applied mathematics, probability, economy and geography \citep{villani2008optimal, carlier2012optimal,gross2016recent}. Specifically, we consider two sets of $d$-dimensional data, which are generated from two different distributions denoted by $X\sim\mu$ and $Y\sim\nu$.\footnote{The optimal transport can also handle more than two distributions. See Section \ref{sec:framework} for more details.} We aim to find an optimal joint distribution $\gamma$ of $X$ and $Y$, which minimizes the expectation on some cost function $c$, i.e., 
\begin{align}
\label{eq:intro}
\gamma^*= \argmin_{\gamma \in \Pi(\mu,\nu)} \mathbb{E}_{(X,Y)\sim \gamma} [c(X,Y)],
\end{align}
The constraint $\gamma \in \Pi(\mu,\nu)$ requires the marginal distribution of $X$ and $Y$ in $\gamma$ to be identical to $\mu$ and $\nu$, respectively. Existing literature often refers to the optimal expected cost $\mathcal{W}^*(\mu,\nu)=\mathbb{E}_{(X,Y)\sim \gamma^*} [c(X,Y)]$ as \textit{Wasserstein distance}, and $\gamma^*$ as the \textit{optimal transport plan}. For domain adaptation, the function $c$ measures the discrepancy between $X$ and $Y$, and the optimal transport plan $\gamma^*$ essentially reveals the transfer of the knowledge from source $X$ to target $Y$. For resource allocation, the function $c$ is the cost of assigning resource $X$ to receiver $Y$, and the optimal transport plan $\gamma^*$ essentially yields the optimal assignment.

%Despite of the imperative need of the optimal transport in many applications, 
Since \eqref{eq:intro} is an optimization problem over the space of distributions, the problem is infinite dimensional and generally intractable when $\mu$ and $\nu$ are continuous distributions.
%Note that \eqref{eq:intro} is actually an optimization problem over the space of distributions. When $\mu$ and $\nu$ are continuous distributions, such a problem is essentially infinite dimensional and generally intractable. 
Therefore, existing literature has resorted to finite dimensional approximations. For example, \citet{cuturi2013sinkhorn} propose to discretize the support using a refined grid, and cast \eqref{eq:intro} into a finite dimensional linear programming problem. However, for complex distributions in high dimensions (e.g., images in domain adaptation), the grid size often needs to be exponentially large (e.g., exponential in dimension) to ensure a small approximation error (due to discretization). Under such a regime, conventional linear programming algorithms do not scale well, e.g., the interior point method in conjunction with the Newton's method takes ${\cO}(n^3 \log n)$ time, where $n$ is the grid size. To ease such a scalability issue, \citet{cuturi2013sinkhorn} propose an entropy regularization-based Sinkhorn algorithm, which requires the computational cost of ${\cO}(n^2)$, but still fail to scale to large problems. 

While there exist several scalable stochastic algorithms for computing Wasserstein distance for continuous distributions $\mu$ and $\nu$ \citep{genevay2016stochastic, seguy2017large, yang2018scalable}, they cannot compute the optimal transport plan $\gamma^*$ (see Section \ref{sec:discussion} for more discussion), which is crucial in the aforementioned applications. 
%We remark that there exist several scalable stochastic algorithms for computing Wasserstein distance for continuous distributions $\mu$ and $\nu$. All these methods can compute $\mathcal{W}^*(\mu,\nu)$, however, they cannot compute the optimal transport plan $\gamma^*$ (see Section \ref{sec:discussion} for more discussion), which is crucial in the aforementioned applications. 

%Therefore, they cannot be readily applied to the aforementioned applications.

%Besides computation issues, the large grid size for discretization also leads to the curse of dimensionality in statistical recovery. Since we can only access finite data from $\mu$ and $
%\nu$ in practice, the large grid size actually needs a huge sample size (e.g., exponential in dimension) to guarantee an accuracy estimator of $\gamma^*$.

To address the scalability and efficiency issues, we propose a new implicit generative learning-based framework for solving optimal transport problems. Specifically, we approximate $\gamma^*$ by a generative model, which maps from some latent variable $Z$ to $(X,Y)$. For simplicity, we denote
\begin{align}\label{nn-generator}
\left[
\begin{array}{c}
X\\
\hline
Y
\end{array}
\right]
=G(Z)=\left[
\begin{array}{c}
G_X(Z)\\
\hline
G_Y(Z)
\end{array}
\right]\quad\textrm{with}\quad Z\sim\rho,
\end{align}
where $\rho$ is some simple latent distribution and $G$ is some operator, e.g., deep neural network or neural ordinary differential equation (ODE).
Accordingly, instead of directly estimating the probability density of $\gamma^*$, we estimate the mapping $G$ between $Z$ and $(X,Y)$ by solving
\begin{align}\label{generative-learning}
G^*=~&\argmin_G \quad~~ \EE_{Z\sim\rho}[c(G_X(Z),G_{Y}(Z))], \quad \textrm{subject~to}\quad G_{X}(Z)\sim\mu,~G_{Y}(Z)\sim\nu
\end{align}
We then cast \eqref{generative-learning} into a minimax optimization problem using the Lagrangian multiplier method. As the constraints in \eqref{generative-learning} are over the space of continuous distributions, the Lagrangian multiplier is actually infinite dimensional. Thus, we propose to approximate the Lagrangian multiplier by deep neural networks, which eventually delivers a finite dimensional generative learning problem. 


Our proposed framework has three major benefits: (1) Our formulated minimax optimization problem can be efficiently solved by primal dual stochastic gradient-type algorithms. Many empirical studies have corroborated that these algorithms can easily scale to very large minimax problems in machine learning \citep{brock2018large}; (2) Our framework can take advantage of recent advances in deep learning. Many empirical evidences have suggested that deep neural networks can effectively adapt to data with intrinsic low dimensional structures \citep{zhang2016understanding, li2018measuring}. Although they are often overparameterized, due to the inductive biases of the training algorithms, the intrinsic dimensions of deep neural networks are usually controlled very well, which avoids the curse of dimensionality; (3) Our adopted generative models allow us to efficiently sample from the optimal transport plan. This is very convenient for certain downstream applications such as domain adaptation, where we can generate infinitely many data points paired across domains \citep{liu2016coupled}.

Moreover, the proposed framework can also recover the density of entropy regularized optimal transport plan.
Specifically, we adopt the neural Ordinary Differential Equation (ODE) approach in \citet{chen2018neural} to model the dynamics that how $Z$ gradually evolves to $G(Z)$.  
 We then derive the ODE that describes how the density evolves, and solve the density of the transport plan from the ODE.  The recovery of density requires no extra parameters, and can be evaluated efficiently. 


%\cite{dai2017calibrating} and  is optimized over the Lagrangian dual 
%Since the marginal constrain of \eqref{eq:intro} is infinite dimensional, the Lagrangian multiplier is also infinite dimensional.
%Parametrized by neural network, the Lagrangian multiplier is constrained to be Lipchitz-$\eta$ function, where $\eta$ is a tuning parameter, to avoid numerical problem caused by possibly not completely satisfied constrain due to the limitation in the complexity of NN.
%This is to avoid numerical problem caused by not completely satisfied constrain and infeasible minimax problem limited by the complexity of NN.
%Limited by the complexity of NN, the equality constrain is usually not satisfied completely, and therefore the minimax problem is not feasible.   

%First, our formulation allows for alternative gradient descent optimization with mini-batches, and therefore is scalable to number of samples. Second, recent advances in theoretical research of deep learning show deep neural networks are automatically adaptive to the dimension of the data. This allows us to easily tune the hyper-parameters with over-parametrization. Third, the formulation of generative model allows for efficient sampling from the transport plan. In applications like domain adaptation, this means we can generate unlimited number of paired data, which is beneficial for downstream application as .

%The rest of this paper is organized as follows: Section 2 briefly introduces background knowledge of optimal transport and implicit generative learning; Section 3 proposes the new computational framework; Section 4 discusses how we convert an implicit generative model to an explicit optimal transportation plan; Section 5 presents detail experimental results on both synthetic and real data; Section 6 discusses the related works; Section 7 draws a brief conclusion.

\noindent {\bf Notations}: 
Given a matrix $A\in\RR^{d\times d}$, $\det(A)$ denotes its determinant, $\tr(A)=\sum_{i}A_{ii}$ denotes its trace, $\norm{A}_{\rm F}=\sqrt{\sum_{i, j}A_{ij}^2}$ denotes its Frobenius norm, and $|A|$ denotes a matrix with $[|A|]_{ij}=|A_{ij}|$. We use  $\textrm{dim}(v)$ to denote the dimension of a vector $v$.














==> Tech_Report copy/method.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

%\begin{figure}[!htb]
%\centering
%%\vspace{-0.in}
%\includegraphics[width=0.35\textwidth]{figures/arche.pdf}
%%\vspace{-0.15in}
%\caption{\label{fig:arche} \it An illustrative example of SPOT framework.}
%%\vspace{-0.1in}
%\end{figure}

\begin{wrapfigure}{r}{0.52\textwidth}
  \begin{center}
  \vspace{-20pt}
    \includegraphics[width=0.48\textwidth]{figures/arche.pdf}
  \end{center}
  \caption{\label{fig:arche}  An illustration of SPOT. }
  \vspace{-20pt}
\end{wrapfigure}

%\vspace{-0.15in}
\section{Scalable OT with Pushforward}\label{sec:framework}
%\vspace{-0.05in}


To achieve better efficiency and scalability, we propose a new framework --- named SPOT (Scalable Pushforward of Optimal Transport) --- for solving the optimal transport problem. 
%Before we proceed with the derivation, we first introduce some notations and assumptions. 
Recall that we aim to find an optimal joint distribution $\gamma$ given by \eqref{eq:intro}. 
Let $\cW_1(X,\mu)$ denotes the standard Wasserstein metric between a random vector $X$ and a distribution $\mu$. Specifically, we write
\begin{align*}
\cW_1(X,\mu) &= \sup_{\lambda_X\in\cF^{1}}\EE_X[\lambda_X(X)] -\mathbb{E}_{U\sim \mu}[\lambda_X(U)],
%\cW_1(Y,\mu) &= \sup_{\lambda_Y\in\cF^1}\EE_Y[\lambda_Y(Y)] -\mathbb{E}_{V\sim \mu}[\lambda_Y(V)],
\end{align*}
where $\cF^{1}$ denotes the class of all $1$-Lipschitz functions from $\RR^d$ to $\RR$. Note that $\cW_1(X,\mu)=0$ indicates $X\sim \mu$. Let $\cW_1(Y,\nu)$ be defined analogously as $\cW_1(X,\mu)$. Then we can rewrite \eqref{eq:intro} as
\begin{align}\label{eq:intro:wasserstein}
\gamma^*= \argmin_{\gamma}~\mathbb{E}_{(X,Y)\sim \gamma} [c(X,Y)], \quad \textrm{subject~to}~\quad \cW_1(X,\mu)=0,~\cW_1(Y,\nu) = 0.
\end{align}
As mentioned earlier, solving $\gamma$ in the space of all continuous distributions is generally intractable. Thus, we adopt the push-forward method, which introduces a mapping $G$ from some latent variable $Z$ to $(X, Y)$. Recall that we denote $(X, Y) = G(Z) = (G_X(Z), G_Y(Z))$ as shown in \eqref{nn-generator}. The latent variable $Z$ follows some distribution $\rho$ that is easy to sample. By the Lagrangian multiplier method and the Kantorovich-Rubinstein duality \citep{villani2008optimal}, we then rewrite \eqref{eq:intro:wasserstein} as
\begin{align}
\min_{G} & \max_{\eta_X,\eta_Y,\lambda_{X}\in\cF^1, \lambda_{Y}\in\cF^{1}}   \mathbb{E}_{Z\sim \rho} [c(G_X (Z),G_Y (Z))] \nonumber \\
& \qquad \quad + \eta_X\mathbb{E}_{Z\sim \rho} [\lambda_X(G_X (Z))] -\mathbb{E}_{U\sim \mu}[\lambda_X(U)]   
 + \eta_Y\mathbb{E}_{Z\sim \rho} [\lambda_Y(G_Y (Z))] -\mathbb{E}_{V\sim \nu}[\lambda_Y(V)]. \label{eq:objective}
\end{align}
Motivated by \citet{arjovsky2017wasserstein}, we then further parameterize $G$, $\lambda_X$, and $\lambda_Y$ with neural networks\footnote{Using a single neural network to parameterize $G$ encourages parameter sharing between $G_X$ and $G_Y$. In fact, we can also parameterize $G_X$ and $G_Y$ with different neural networks.}. We denote $\cG$ as the class of neural networks for parameterizing $G$ and similarly $\cF_X^{1}$ and $\cF_Y^{1}$ as the classes of $1$-Lipschitz functions for $\lambda_X$ and $\lambda_Y$, respectively. 
%By such a parameterization, we cast \eqref{eq:objective} into a finite dimensional minimax optimization problem.

%obtain the following finite dimensional minmax optimization problem
%\begin{align}
%\min_{G\in \mathcal{G}} & \max_{\lambda_{X} \in \mathcal{F}_X, \lambda_{Y} \in \mathcal{F}_Y} \mathbb{E}_{Z\sim \rho} [c(G_{X} (Z),G_{Y} (Z))] \notag \\
%&\quad + \mathbb{E}_{Z\sim \rho} [\lambda_{X}(G_{X} (Z))] -\mathbb{E}_{X\sim \mu}[\lambda_{X}(X)]  \notag \\
%&\quad + \mathbb{E}_{Z\sim \rho} [\lambda_{Y}(G_{Y} (Z))] -\mathbb{E}_{Y\sim \nu}[\lambda_{Y}(Y)]. \label{eq:finiteobjective}
%\end{align}
Since $\cG$, $\cF_X$, and $\cF_Y$ are only finite classes, our parameterization of $G$ cannot exactly represent any continuous distributions of $(X,Y)$ (only up to a small approximation error with sufficiently many neurons). Then the marginal distribution constraints, $G_X(Z) \sim \mu$ and $G_Y(Z) \sim \nu$, are not necessarily satisfied. Therefore, the Lagrangian multipliers can be unbounded and the equilibrium of \eqref{eq:objective} does not necessarily exist. To address this issue, we directly treat $\eta_X=\eta_Y=\eta$ as tuning parameters, and solve the following problem instead
\begin{align}
\min_{G\in \mathcal{G}}  \max_{\lambda_{X}\in \mathcal{F}_{X}^{1}, \lambda_{Y} \in \mathcal{F}_{Y}^{1}} & \mathbb{E}_{Z\sim \rho} [c(G_{X} (Z),G_{Y} (Z))] \notag \\
& + \eta\big(\mathbb{E}_{Z\sim \rho} [\lambda_{X}(G_{X} (Z))] -\mathbb{E}_{X\sim \mu}[\lambda_{X}(X)] 
+ \mathbb{E}_{Z\sim \rho} [\lambda_{Y}(G_{Y} (Z))] -\mathbb{E}_{Y\sim \nu}[\lambda_{Y}(Y)]\big). \label{eq:finalvariant}
\end{align}
We apply alternating stochastic gradient algorithm to solve \eqref{eq:finalvariant}: in each iteration, we perform a few steps of gradient ascent on $\lambda_X$ and $\lambda_Y$, respectively for a fixed $G$, followed by one-step gradient descent on $G$ for fixed $\lambda_X$ and $\lambda_Y$. We use Spectral Normalization (SN, \citet{miyato2018spectral}) to control the Lipschitz constant of $\lambda_X$ and $\lambda_Y$ being smaller than 1. Specifically, SN constrains the spectral norm of each weight matrix $W$ by $\textrm{SN}(W) = W / \sigma(W)$ in every iteration, where $\sigma(W)$ denotes the spectral norm of $W$. Note that $\sigma(W)$ can be efficiently approximated by a simple one-step power method \citep{golub2001eigenvalue}. Therefore, the computationally intensive SVD can be avoided. We summarize the algorithm in Algorithm \ref{alg1} with SN omitted.% where SN is contained in the parametrization of $\lambda_X$ and $\lambda_Y$. 
%we slightly abuse the notation to denote SN of weight matrices for a network parameterized with $\theta$ by $\textrm{SN}(\theta)$.

\setlength{\textfloatsep}{2pt}
\vspace{-0.1in}
\begin{algorithm}[h]
\caption{Mini-batch Primal Dual Stochastic Gradient Algorithm for SPOT} 
\label{alg1}
\begin{algorithmic} 
    \REQUIRE Datasets $\{x_i\}_{i=1}^N\sim \mu, \{y_j\}_{j=1}^M\sim \nu$; Initialized networks $G$, $\lambda_X$, and $\lambda_Y$ with parameters $w$,  $\theta$, and $\beta$, respectively; $\alpha$, the learning rate; $n_{\rm{critic}}$, the number of gradient ascent for $\lambda_X$ and $\lambda_Y$; $n$, the batch size
    \WHILE{$w$ not converged}
        \FOR{$t=1,2,\cdots,n_{\rm{critic}}$}
        \STATE Sample mini-batch $\{x_i\}_{i=1}^n$ from $\{x_i\}_{i=1}^N$
        \STATE Sample mini-batch $\{y_j\}_{j=1}^n$ from $\{y_j\}_{j=1}^M$
        \STATE Sample mini-batch $\{z_k\}_{k=1}^n$ from $\rho$
        \STATE $g_{\theta} \leftarrow  \nabla_{\theta} (\eta\frac{1}{n}\sum_{k=1}^n \lambda_{X,\theta}(G_{X,w} (z_k))$\\\hspace{3.5cm}$ -\eta\frac{1}{n}\sum_{i=1}^n\lambda_{X,\theta}(x_i) )$
        \STATE $g_{\beta} \leftarrow  \nabla_{\beta} (\eta\frac{1}{n}\sum_{k=1}^n \lambda_{Y,\beta}(G_{Y,w} (z_k))$\\\hspace{3.5cm}$ -\eta\frac{1}{n}\sum_{i=1}^n\lambda_{Y,\beta}(y_i) )$
        \STATE $\theta \leftarrow \theta + \alpha g_{\theta}$, $\beta \leftarrow \beta + \alpha g_{\beta}$
%        \STATE $\theta \gets \rm{SN}(\theta)$, $\beta \gets \rm{SN}(\beta)$
        \ENDFOR
        \STATE Sample mini-batch $\{z_k\}_{k=1}^n$ from $\rho$
        \STATE $g_{w} \leftarrow  \nabla_{w} (\frac{1}{n}\sum_{k=1}^n c(G_{X,w} (z_k),G_{Y,w} (z_k))$
        \\\hspace{2cm}$ + \eta\frac{1}{n}\sum_{k=1}^n \lambda_{X,\theta}(G_{X,w} (z_k)) $
        \\\hspace{3.2cm}$+ \eta\frac{1}{n}\sum_{k=1}^n \lambda_{Y,\beta}(G_{Y,w} (z_k))$
        \STATE $w \leftarrow w + \alpha g_w$
    \ENDWHILE
\end{algorithmic}
\end{algorithm}

%we force the Lipchitz constraint by spectral  normalization. Spectral  normalization forces functions $\lambda_X$ and $\lambda_Y$ to be 1-Lipchitz continuous. We then multiplies functions $\lambda_X$ and $\lambda_Y$ by a tunable constant $\eta$, to scale them so that their Lipchitz constant is suitable for the problem. In this way, we have a refined control of the constraint violation by tuning $\kappa$. Finally, our objective function is
%\begin{align}
%\min_{G\in \mathcal{G}} & \max_{\lambda_{X}\in \mathcal{F}_{X}^{(r)}, \lambda_{Y} \in \mathcal{F}_{Y}^{(r)}}   \mathbb{E}_{Z\sim \rho} [c(G_X (Z),G_Y (Z))]\notag \\
%&+ \eta \large( \mathbb{E}_{Z\sim \rho} [\lambda_X(G_X (Z))] -\mathbb{E}_{X\sim \mu}[\lambda_X(X)] \notag \\
%&+ \mathbb{E}_{Z\sim \rho} [\lambda_Y(G_Y (Z))] -\mathbb{E}_{Y\sim \nu}[\lambda_Y(Y)] \large).\label{eq:finalobjective}
%\end{align}
%Denote the objective function in \eqref{eq:finalobjective} as $\cL$. Note that unlike \eqref{eq:finalobjective1}, the products $\eta\lambda_X$, and $\eta\lambda_Y$ serves as the Lagrangian multiplier in \eqref{eq:finalobjective}.
%The above minimax problem can be optimized by alternating gradient descent over $G$ and $\lambda_{X}$, $\lambda_{Y}$. In each iteration, fixing $G$, we perform gradient ascent over $\lambda_{X}$, $\lambda_{Y}$. After the gradient ascent converges, we perform one step of gradient descent over $G$ with fixed $\lambda_{X}$, $\lambda_{Y}$.  Algorithm \ref{alg1} shows the algorithm of SPOT with vanilla stochastic gradient descent (SGD), while other more complicated optimization algorithm \citep{kingma2014adam, ruder2016overview} can also be applied in our case. 
%\begin{algorithm} 
%\caption{Implicit generative model training} 
%\label{alg1}
%\begin{algorithmic} 
%    \REQUIRE $\{x_i\}_{i=1}^N\sim \mu, \{y_j\}_{j=1}^M\sim \nu$
%    \REQUIRE Initialized networks $G$, $\lambda_X$ and $\lambda_Y$ with parameters $w$,  $\theta$ and $\beta$, respectively; $\alpha$, the learning rate
%    \WHILE{$w$ not converged}
%        \WHILE{$\theta$, $\beta$ not converged}
%        \STATE Sample mini-batch $\{x_i\}_{i=1}^n$ from $\{x_i\}_{i=1}^N$
%        \STATE Sample mini-batch $\{y_j\}_{j=1}^n$ from $\{y_j\}_{j=1}^M$
%        \STATE Sample mini-batch $\{z_k\}_{k=1}^n$ from $\rho$
%        \STATE $g_{\theta} \leftarrow  \nabla_{\theta} (\eta\frac{1}{n}\sum_{k=1}^n \lambda_{X,\theta}(G_{X,w} (z_k))$\\\hspace{3.5cm}$ -\eta\frac{1}{n}\sum_{i=1}^n\lambda_{X,\theta}(x_i) )$
%        \STATE $g_{\beta} \leftarrow  \nabla_{\beta} (\eta\frac{1}{n}\sum_{k=1}^n \lambda_{Y,\beta}(G_{Y,w} (z_k))$\\\hspace{3.5cm}$ -\eta\frac{1}{n}\sum_{i=1}^n\lambda_{Y,\beta}(y_i) )$
%        \STATE $\theta \leftarrow \theta + \alpha g_{\theta}$, $\beta \leftarrow \beta + \alpha g_{\beta}$
%        \STATE $\theta = \rm{SN}(\theta)$,$\beta = \rm{SN}(\beta)$
%        \ENDWHILE
%        \STATE Sample mini-batch $\{z_k\}_{k=1}^n$ from $\rho$
%        \STATE $g_{w} \leftarrow  \nabla_{w} (\frac{1}{n}\sum_{k=1}^n c(G_{X,w} (z_k),G_{Y,w} (z_k))$
%        \\\hspace{2cm}$ + \eta\frac{1}{n}\sum_{k=1}^n \lambda_{X,\theta}(G_{X,w} (z_k)) $
%        \\\hspace{3.2cm}$+ \eta\frac{1}{n}\sum_{k=1}^n \lambda_{Y,\beta}(G_{Y,w} (z_k))$
%        \STATE $w \leftarrow w + \alpha g_w$
%    \ENDWHILE
%\end{algorithmic}
%\end{algorithm}
%We can absorb $\eta$ into the multipliers $\lambda_X$ and $\lambda_Y$ such that $\eta\lambda_X$ and $\eta\lambda_Y$ are $\eta$-Lipschitz, which adds more flexibility to control the influence of $G_X$ and $G_Y$ being possibly infeasible. In fact, with fine tuned parameter $\eta$, we can achieve
%\begin{align*}
%\cR = &~\mathbb{E}_{Z\sim \rho} [\lambda_{X}(G_{X} (Z))] -\mathbb{E}_{X\sim \mu}[\lambda_{X}(X)] \\
%&+ \mathbb{E}_{Z\sim \rho} [\lambda_{Y}(G_{Y} (Z))] -\mathbb{E}_{Y\sim \nu}[\lambda_{Y}(Y)]
%\end{align*}
%very small (see more details in Section \ref{section51}).
%The above formula is a minimax problem where we seek to solve $p_{\gamma}^* $, i.e. the density of optimal transport plan. As aforementioned, directly density estimation might not be intractable of inefficient. Therefore, instead of solving for $p_{\gamma}$ directly, we adopt push-forward based method.
%Specifically, our goal is to train a mapping that takes a latent random variable $Z\sim \rho$ as input, and outputs a tuple of random variables $G_{\mathcal{X}}(Z),G_{\mathcal{Y}}(Z)$, i.e.
%\begin{align*}
%G: &\mathcal{Z}\to \mathcal{X}\times \mathcal{Y}\\
%& Z \mapsto G(Z)  = (G_X(Z),G_Y(Z)),
%\end{align*}
%where $G_X(Z),G_Y(Z)$ are the components of $G(Z)$ in space $\mathcal{X}$ and $\mathcal{Y}$, respectively. 
%We use the , i.e. 
%In this way, since we can get the samples of $\gamma$ by feed samples of $Z$ into $G(\cdot)$, the integrations in above equation can be rewritten into the expectations of samples. Therefore, replacing $\gamma$ with distribution of $G(Z)$, the minimax problem can be rewritten as
%\begin{align}
%\min_{G} & \max_{\lambda_{\mathcal{X}}, \lambda_{\mathcal{Y}} }   \mathbb{E}_{Z\sim \rho} [c(G_X (Z),G_Y (Z))] \nonumber \\
%&+ \mathbb{E}_{Z\sim \rho} [\lambda_X(G_X (Z))] -\mathbb{E}_{X\sim \mu}[\lambda_X(X)]   \nonumber \\
%&+ \mathbb{E}_{Z\sim \rho} [\lambda_Y(G_Y (Z))] -\mathbb{E}_{Y\sim \nu}[\lambda_Y(Y)] . \label{eq:objective}
%\end{align}
%
%In the above formula, the optimization variable $G$, $\lambda_{X}(\cdot)$, and $\lambda_{Y}(\cdot)$ are  infinite dimensional. 
%We parametrize $G(\cdot)$, $\lambda_{X}(\cdot)$, and $\lambda_{Y}(\cdot)$ as three neural networks. The two part of $G(\cdot)$, i.e., $G_{X}(\cdot)$ and $G_{Y}(\cdot)$, might either have shared parameters or might not. 
%By parametrization the functions with finite amount of parameters, we actually restrict function $G(\cdot)$ to be in a space $\cG$, functions $\lambda_{X}(\cdot)$, and $\lambda_{Y}(\cdot)$ to be in space $\cF$. The space $\mathcal{G}$ and $\mathcal{F}$ we pick can only have finite complexity, but the equality constrain has infinite dimension. As a consequence, the minimax problem might not be feasible, and thus the equality constrain might not be completely satisfied. If so, the optimal $\lambda_{X}(\cdot)$, and $\lambda_{Y}(\cdot)$ of the minimax problem would blow up. 
%
%To address this issue, we modify the objective function \eqref{eq:objective} by constraining $\lambda_{\mathcal{X}}$ and $\lambda_{\mathcal{Y}}$ to be Lipchitz-1 functions, and adding tuning parameter $\eta$ as the scaling factor,
%\begin{align*}
%\min_{G\in \mathcal{G}}\max_{\lambda_{\mathcal{X}}, \lambda_{\mathcal{X}} \in \mathcal{F}_1}  & \mathbb{E}_{Z\sim \rho} [c(G_{\mathcal{X}} (Z),G_{\mathcal{Y}} (Z))] \\
%&+ \eta \large( \mathbb{E}_{Z\sim \rho} [\lambda_{\mathcal{X}}(G_{\mathcal{X}} (Z))] -\mathbb{E}_{X\sim \mu}[\lambda_{\mathcal{X}}(X)]  \\
%&+ \mathbb{E}_{Z\sim \rho} [\lambda_{\mathcal{Y}}(G_{\mathcal{Y}} (Z))] -\mathbb{E}_{Y\sim \nu}[\lambda_{\mathcal{Y}}(Y)] \large),
%\end{align*}
%where the Lipchitz constrain is enforced following \cite{arjovsky2017wasserstein}. In the above formula, the Lagrangian multipliers are essentially $\eta\lambda_{\cX}$ and $\eta\lambda_{\cX}$, so we essentially constrain the multiplier to be Lipchitz-$\lambda$. 
%In this way, $f_{\mathcal{X}}$ and $f_{\mathcal{Y}}$ form the \textit{neural distances} \cite{arora2017generalization} between distributions of $G_{\mathcal{X}}(Z)$ and $X$, $G_{\mathcal{Y}}(Z)$ and $Y$, respectively, and good generalization properties are guaranteed as a consequence. 
%With proper choice of $\lambda$, the term
%\begin{align*}
%\cR = &\mathbb{E}_{Z\sim \omega} [\lambda_{\mathcal{X}}(G_{\mathcal{X}} (Z))] -\mathbb{E}_{X\sim \mu}[\lambda_{\mathcal{X}}(X)] \\
%&+ \mathbb{E}_{Z\sim \omega} [\lambda_{\mathcal{Y}}(G_{\mathcal{Y}} (Z))] -\mathbb{E}_{Y\sim \nu}[\lambda_{\mathcal{Y}}(Y)]
%\end{align*} 
%can be very small, as we will show in experiments.  
%
%In the following lemma, we show that the difference between computed Wasserstein distance $\mathcal{\hat{W}}(\mu,\nu)=\mathbb{E}_{Z\sim \omega} [c(G_{\mathcal{X}} (Z),G_{\mathcal{Y}} (Z))]$ with optimal $G$ and the true Wasserstein distance $\mathcal{W}(\mu,\nu)$ is bounded by this small value.
%\begin{remark}
%When restricting $\lambda_X$ to be $1$-Lipschitz functions, the term $\mathbb{E}_{Z\sim \rho} [\lambda_{X}(G_{X} (Z))] -\mathbb{E}_{X\sim \mu}[\lambda_{X}(X)]$ is essentially the Wasserstein distance between the distributions of $G_X(Z)$ and $Z$ under the Euclidean ground cost \citep{villani2008optimal}. Thus, the proposed objective function \eqref{eq:finalobjective} is consistent with the relaxed Kantorovich formulation \citep{liero2018optimal, chizat2015unbalanced}, when the divergences of marginal distributions are chosen to be the Wasserstein distance. 
%\end{remark}
%\vspace{-0.05in}
{\bf Connection to Wasserstein Generative Adversarial Networks (WGANs)}:
Our proposed framework \eqref{eq:finalvariant} can be viewed as a multi-task learning version of Wasserstein GANs \citep{liu2016coupled, liu2018multi}. Specifically, the mapping $G$ can be viewed as a \textit{generator} that generates samples in the domains $\cX$ and $\cY$. The Lagrangian multipliers $\lambda_X$ and $\lambda_Y$ can be viewed as \textit{discriminators} that evaluate the discrepancies of the generated sample distributions and the target marginal distributions. By restricting $\lambda_X \in \cF_X^1$, $\mathbb{E}_{Z\sim \rho} [\lambda_{X}(G_{X} (Z))] -\mathbb{E}_{X\sim \mu}[\lambda_{X}(X)]$ essentially approximates the Wasserstein distance between the distributions of $G_X(Z)$ and $X$ under the Euclidean ground cost (\citet{villani2008optimal}, the same holds for $Y$). Denote 
\begin{align*}
& \cR(G_X, G_Y) = \mathbb{E}_{Z\sim \rho} [c(G_{X} (Z),G_{Y} (Z))], \quad \textrm{and} 
& d_{w}(G_X, X) = \max_{\lambda_X \in \cF_X^1} \mathbb{E}_{Z\sim \rho} [\lambda_X(G_{X} (Z))] -\mathbb{E}_{X\sim \mu}[\lambda_{X}(X)].
\end{align*}
Let $d_w(G_Y, Y)$ be defined analogously as $d_w(G_X, X)$. We can rewrite \eqref{eq:finalvariant} as
\begin{align}
\label{eq:multi-gan}
\min_{G \in \cG} \eta\big(d_{w}(G_X, X) + d_{w}(G_Y, Y)\big) + \cR(G_X, G_Y),
\end{align}
which essentially learns two Wasserstein GANs with a joint generator $G$ through the regularizer $\cR$. An illustrative example is provided in Figure \ref{fig:arche}.



%Thus, by solving \eqref{eq:finalobjective}, we not only obtain generated samples $G_X(Z)$ and $G_Y(Z)$ that mimic the two target marginal distributions, but also provide the optimal transport plan that can be computed from $G$.

%Therefore, the proposed objective function can be viewed as two scaled Wasserstein generative adversarial loss functions for marginals $X$ and $Y$, respectively, plus an regularization term to promote the optimal transport relationship between the two marginals. As can be seen, by solving \eqref{eq:finalobjective}, we can not only provide the samples that mimic the data from the two input datasets, but also offers the optimal joint distribution of them in the sense of optimal transport. 

%\vspace{-0.05in}
{\bf Extension to Multiple Marginal Distributions}:
Our proposed framework can be straightforwardly extended to more than two marginal distributions. Consider the ground cost function $c$ taking $m$ inputs $X_1, \dots, X_m$ with $X_i \sim \mu_i$ for $i = 1, \dots, m$. Then the optimal transport problem \eqref{eq:intro} becomes the multi-marginal problem \citep{pass2015multi}:
\begin{align}
\gamma^*= \argmin_{\gamma \in \Pi(\mu_1, \mu_2,\cdots, \mu_m)} \mathbb{E}_{\gamma} [c(X_1,X_2,\cdots, X_m)], \label{eq:multidist}
\end{align}
where $\Pi(\mu_1, \mu_2,\cdots, \mu_m)$ denotes all the joint distributions with marginal distributions satisfying $X_i \sim \mu_i$ for all $i = 1, \dots, m$. Following the same procedure for two distributions, we cast \eqref{eq:multidist} into the following form
\begin{align*}
\min_{G\in \mathcal{G}} & \max_{\lambda_{X_i}\in \mathcal{F}_{X_i}^{\eta}} \mathbb{E}_{Z\sim \rho} [c(G_{X_1} (Z),\cdots, G_{X_m} (Z))]   + \textstyle\sum_{i=1}^m \left(\mathbb{E}_{Z\sim \rho} [\lambda_{X_i}(G_{X_i} (Z))] -\mathbb{E}_{X_i\sim \mu_i}[\lambda_{X_i}(X_i)] \right),
\end{align*}
where $G$ and $\lambda_{X_i}$'s are all parameterized by neural networks. Existing methods for solving the multi-marginal problem \eqref{eq:multidist} suggest to discretize the support of the joint distribution using a refined grid. For complex distributions, the grid size needs to be very large and can be exponential in $m$ \citep{villani2008optimal}. Our parameterization method actually only requires at most $2m$ neural networks, which further corroborates the scalability and efficiency of our framework.



%is defined to measure distance between more than two points, the Kantorovich formulation can be naturally generalize to multi-marginal case \citep{pass2015multi}. For example, if we have $m$ distribution $\mu_1, \mu_2,\cdots, \mu_m$, the optimal transport plan can be solved by the following optimization problem
%\begin{align}
%\label{eq:kant_multi}
%\gamma^*= \argmin_{\gamma \in \Pi(\mu_1, \mu_2,\cdots, \mu_m)} \mathbb{E}_{(X_1,\cdots, X_m)\sim \gamma} [c(X_1,X_2,\cdots, X_m)],
%\end{align}
%where the marginal distribution of $X_i$ in $\gamma$ is identical to $\mu_i$. In this case, the objective function \eqref{eq:finalobjective} rewritten as
%\begin{align*}
%\min_{G\in \mathcal{G}} & \max_{\lambda_{X_i}\in \mathcal{F}_{X_i}^{\eta}} \mathbb{E}_{Z\sim \rho} [c(G_{X_1} (Z),G_{X_2} (Z),\cdots, G_{X_m} (Z))]  \\
%&\quad + \sum_{i=1}^m \left(\mathbb{E}_{Z\sim \rho} [\lambda_{X_i}(G_{X_i} (Z))] -\mathbb{E}_{X_i\sim \mu_i}[\lambda_{X_i}(X_i)] \right). 
%\end{align*}
%Note that  \eqref{eq:kant_multi} with general cost function need to discretize the support of $\gamma$, which leads to a linear program where the number of variables grows exponentially in $m$ \citep{villani2008optimal}. In contrast, the number of parameters in our proposed framework {\color{red} scales approximately linearly with respect to $m$}, which is another aspect of the good scalability of SPOT.


==> Tech_Report copy/special_case.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

%\vspace{-0.15in}
\section{SPOT for Regularized Density Recovery}
\label{section4}
%\vspace{-0.05in}

Existing literature has shown that entropy-regularized optimal transportation outperforms the un-regularized counterpart in some applications \citep{erlander1990gravity, cuturi2013sinkhorn}. This is because the entropy regularizer can tradeoff the estimation bias and variance by controlling the smoothness of the density function.

We demonstrate how to efficiently recover the density $p_\gamma$ of the transport plan with entropy regularization.
%When $\dim(\mathcal{Z})=\dim(\mathcal{X})+\dim(\mathcal{Y})$, and assume the the density of the joint distribution $p(X,Y)$ exists. 
%By change of variable, we can rewrite $p_\gamma$ as
%\begin{align}
%\label{eq:change_variable}
%    p_{\gamma} (G_X(Z), G_Y(Z))= p_Z(Z)\left\lvert\det \rbr{\frac{d G(Z)}{d Z}}\right\rvert^{-1},
%\end{align}
%where $p_Z$ is the density of $Z$, and $\frac{dG(Z)}{dZ}$ is the Jacobian matrix of the mapping $G$. %Recall that generative flow methods suggest to decompose $\frac{dG(Z)}{dZ}$ by the product of the Jacobian matrix of each layer in the neural network. By restricting the Jacobian matrix in each layer to be triangular, we can efficiently compute $\det \rbr{\frac{d G(Z)}{d Z}}$ and obtain $p_\gamma$. %the density $p_{\gamma}$ can be either recovered by generative flow methods or neural ordinary equation method. In generative flow methods, the Jacobian matrix  $d G(Z)/d Z$ is computed by chain rule, which, more specifically, is the multiplication of the transition functions' Jacobian matrices. When some sparse structure is enforced in the transition functions' Jacobian matrices, the density $p_{\gamma}$ is easy to compute using formula \eqref{eq:change_variable} \citep{dinh2014nice, kingma2018glow,chen2018neural}.
%Imposing constraints on the neural network for parameterizing $G$, however, deteriorates its approximation power. 
Instead of parameterizing $G$ by a feedforward neural network, we choose the neural ODE approach, which uses neural networks to approximate the transition from input $Z$ towards output $G(Z)$ in the continuous time. Specifically, we take $z(0) = Z$ and $z(1) = G(Z)$. Let $z(t)$ be the continuous interpolation of $Z$ with density $p(t)$ varying according to time $t$. We split $z(t)$ into $z_1(t)$ and $z_2(t)$ such that $\textrm{dim}(z_1) = \textrm{dim}(X)$ and $\textrm{dim}(z_2) = \textrm{dim}(Y)$. We then write the neural ODE as
\begin{align}
\label{eq:ODE}
dz_1/dt=\xi_1(z(t),t), \quad dz_2/dt=\xi_2(z(t),t),
\end{align}
where $\xi_1$ and $\xi_2$ capture the dynamics of $z(t)$. We parameterize $\xi = (\xi_1, \xi_2)$ by a neural network with parameter $w$. %Recall that $\xi_1$ and $\xi_2$ largely simplify the density recovery of $p_\gamma$. Since $G$ involves the above ODEs,
We can describe the dynamics of the joint density $p(t)$ in the following proposition.
%Before we state the corollary for computing $p_\gamma$, we briefly summarize how to train $\xi_1$ and $\xi_2$ using alternative stochastic gradient method. The algorithm follows Algorithm \ref{alg1}, and updating $G$ becomes more complex due to involving neural ODE.
%Note that here $G$ is a function of $\xi$. Thus, we only need to update the parameter $w$, that is, find the gradient $\partial \cL / \partial w$ with $\cL$ being the objective function of \eqref{eq:finalvariant}. The computation of $\partial \cL / \partial w$ is a bit involved and requires an integral with a so-called adjoint variable $a(t) = -\partial \cL/\partial z(t)$. We refer the readers to \citet{chen2018neural} for a complete derivation. We repeat the aforementioned procedure until convergence. 
%We start with randomly initializing $\xi = (\xi_1, \xi_2)$, $\lambda_X$ and $\lambda_Y$ with parameters $w$, $\theta$ and $\beta$, respectively. We set the learning rate to be $\alpha$. With given $\xi_1$ and $\xi_2$, we can solve \eqref{eq:ODE} with $z(0) = Z$ by some well developed methods such as Euler method and Runge-Kutta method \citep{butcher1987numerical, runge1895numerische, kutta1901beitrag}. Then we take $G(Z) = z(1)$ and do one-step gradient descent to update $\lambda_X$ and $\lambda_Y$ (i.e., parameters $\theta$ and $\beta$). Next we update $G$. 
%There are many developed methods to solve ODEs, such as Euler method, Runge-Kutta method \citep{butcher1987numerical, runge1895numerische, kutta1901beitrag}. Here, we treat the ODE solver as a black box, i.e. we do not need to know the inside components of the solver. 
%Denote $\cL$ as the objective function in \eqref{eq:finalobjective}. Recall that in each training iteration in Algorithm \ref{alg1}, we first do gradient ascent on $\lambda_X$ and $\lambda_Y$. We only need to evaluate the value of $G(Z)$, which can be done by solving ODE \eqref{eq:ODE}. Then we do one step gradient descent on the parameters of $G(\cdot)$, where we need to compute $\partial \cL/\partial w$. Here, the gradient is computed by solving another ODE, instead of naive back-propagation.
%More specifically, the gradient of objective function $\cL$ over parameter $w$ can be written as a integration \citep{chen2018neural}
%\begin{align}
%\label{eq:Lw}
%\frac{d \cL}{d w} = \int_0^1 a(t)^\top \frac{\partial \xi_w(z(t),t)}{\partial w} dt,
%\end{align}
%where $a(t)$ is the adjoint variable $a(t)=-\partial \cL/\partial z(t)$, i.e. how the gradient of the objective function is dependent on the hidden state $z(t)$. Variable $a(t)$ can also be written as an ODE,
%\begin{align}
%\label{eq:at}
%\frac{d a(t)}{d t} = -a(t)^\top \frac{\partial \xi_w(z(t),t)}{\partial z}.
%\end{align}
%The detailed algorithm to compute $\partial \cL/\partial w$ is as follows. First, we solve \eqref{eq:ODE} with initialization $z(0)=Z$, to get $G(Z)=z(1)$, and compute $\cL$. Note that in order to save memory, the computational graph of the procedure does not need to be recorded, since we use \eqref{eq:Lw} to compute the gradient instead of naive automatic differentiation. Then starting from initialization at $t=1$ towards $t=0$, at each time point $t$, we recompute $z(t)$ from \eqref{eq:ODE}, then compute $a(t)$ from \eqref{eq:at}, and compute the inner terms of the integration in \eqref{eq:Lw}. 
%Finally, we average over the inner terms of the integration in \eqref{eq:Lw} in time interval $[0,1]$, which is exactly $\partial \cL/\partial w$.
%Once $\xi$ is trained, we capture the dynamics of the joint density $p_t$ in the following corollary.
\begin{proposition}\label{thm:odep}
%(ODE for the density of transport plan) 
Let $z$, $z_1$, $z_2$, $\xi_1$ and $\xi_2$ be defined as above. Suppose $\xi_1$ and $\xi_2$ are uniformly Lipschitz continuous in $z$ (the Lipschitz constant is independent of $t$) and continuous in $t$. The log joint density satisfies the following ODE:
\begin{equation}\label{eq:prob}
    \frac{\partial \log p(t)}{\partial t} = - \left(\tr \left(\frac{\partial \xi_1}{\partial z_1}\right)+\tr \left(\frac{\partial \xi_2}{\partial z_2}\right)\right),
\end{equation}
where $\frac{\partial \xi_1}{\partial z_1}$ and $\frac{\partial \xi_2}{\partial z_2}$ are Jacobian matrices of $\xi_1$ and $\xi_2$ with respect to $z_1$ and $z_2$, respectively.
\end{proposition}
Proposition \ref{thm:odep} is a direct result of Theorem 1 in \citet{chen2018neural}. We can now recover the joint density by taking $p_\gamma = p(1)$, which further enables us to efficiently compute the entropy regularizer defined as
\begin{align*}
\cH(p_\gamma) = \EE_{G(Z) \sim \gamma} [\log p_{\gamma}(G(Z))].
\end{align*}
Then we consider the entropy regularized Wasserstein distance $\cL_c(G, \lambda_X, \lambda_Y) + \epsilon \cH(p_\gamma)$ where $\cL_c(G, \lambda_X, \lambda_Y)$ is the objective function in \eqref{eq:finalvariant}. Note that here $G$ is a functional operator of $\xi$, and hence parameterized with $w$. The training algorithm follows Algorithm \ref{alg1}, except that updating $G$ becomes more complex due to involving the neural ODE and the entropy regularizer.

To update $G$, we are essentially updating $w$ using the gradient $g_w = \partial (\cL_c + \epsilon \cH) / \partial w$, where $\epsilon$ is the regularization coefficient. First we compute $\partial \cL_c / \partial w$. We adopt the integral form from \citet{chen2018neural} in the following
\begin{align}
\label{eq:Lw}
\frac{\partial \cL_c}{\partial w} = - \int_0^1 a(t)^\top \frac{\partial \xi(z(t),t)}{\partial w} dt,
\end{align}
where $a(t) = \partial \cL_c / \partial z(t)$ is the so-called ``adjoint variable''. The detailed derivation is slightly involved due to the complicated terms in the chain rule.
%\begin{align*}
%\frac{\partial \cL}{\partial w} = \frac{\partial \cL}{\partial z(t)} \frac{\partial z(t)}{\partial w}.
%\end{align*}
We refer the readers to \citet{chen2018neural} for a complete argument. The advantage of introducing $a(t)$ is that we can compute $a(t)$ using the following ODE,
\begin{align*}
%\label{eq:at}
\frac{d a(t)}{d t} = -a(t)^\top \frac{\partial \xi(z(t),t)}{\partial z}.
\end{align*}
Then we can use a well developed numerical method to compute \eqref{eq:Lw} efficiently \citep{davis2007methods}.
%Then we uniformly discretize the interval $[0, 1]$ into $\{t_0, \dots, t_N\}$ and approximate \eqref{eq:Lw} by the finite sum $- \frac{1}{N} \sum_{i=1}^N a(t_i)^\top \frac{\partial \xi(z(t_i),t_i)}{\partial w}$. 
Next, we compute $\partial \cH / \partial w$ in a similar procedure with $a(t)$ replaced by $b(t) = \partial \cH / \partial \log p(t)$. We then write
\begin{align*}
\frac{\partial \cH}{\partial w} = - \int_0^1 b(t)^\top \frac{\partial \log p(t)}{\partial w} dt.
\end{align*}
Using the same numerical method, we can compute $\partial \cH / \partial w$, which eventually allows us to compute $g_w$ and update $w$.

%Instead of recovering the density with a well-trained $\xi$, we compute the density $p_{\gamma}$ in each iteration and impose an entropy regularizer $\cH(p_\gamma)$ to the objective function. Specifically, the entropy regularizer is defined as
%\begin{align*}
%\cH(p_\gamma) = \EE_{(X,Y)\sim \gamma} [\log p_{\gamma}(X,Y)].
%\end{align*}
%At the $t$-th iteration, we recover the density $p_{\gamma, t}$. Then at the $(t+1)$-th iteration, we are essentially optimizing the regularized objective function $\cL + \epsilon \cH(p_{\gamma, t})$ with $\epsilon$ being the regularization coefficient. Entropy regularization has been widely used in optimal transport. 

%add $\epsilon H$ to objective function $\cL$, to achieve a better smoothness of the joint distribution, where $\epsilon$ is the regularization coefficient. In each training step of $G$, we need to compute $\partial (\cL+\epsilon H)/\partial w$, which is dependent on both $z(1)$ and $p_1$. Therefore, we augment the variable $z(t)$ to $[z(t), \log p_t]$, and the gradient can be computed in the same way as above. 
%This entropy regularization is widely used in optimal transport. 
%Existing literature has shown that entropy-regularized optimal transportation outperforms the un-regularized one on some benchmarks \citep{erlander1990gravity, cuturi2013sinkhorn}. The reason behind is that the Wasserstein distance with entropy regularizer tends to have better convexity and smoothness with respect to the input distributions.
%this explicit joint density can be essential to interpretability and downstream tasks [][]. One example of the important use of the explicit value density is to add entropy regularization to Wasserstein distance.  It is reported that entropically regularized optimal transportation outperforms the un-regularized one on some benchmarks \citep{erlander1990gravity, cuturi2013sinkhorn}, since adding entropy would make the Wasserstein distance have better convexity and smoothness with respect to the input distributions.


%As pointed out by \cite{dai2017calibrating}, when an entropy regularizer is added, the discriminator can be interpreted as the scoring function of the generator, providing more stable training and more interpretability. However, in \cite{dai2017calibrating}, the entropy is approximately computed using variational lower bound. Here, with explicit value of density available, the entropy is easily computed exactly.

\vspace{-0.15in}
\section{SPOT for Domain Adaptation}
\vspace{-0.05in}

 Optimal transport has been used in domain adaptation, but existing methods are either computationally inefficient \citep{courty2017joint, damodaran2018deepjdot}, or cannot achieve a state-of-the-art performance \citep{seguy2018large}. Here, we demonstrate that SPOT can tackle large scale domain adaptation problems with state-of-the-art performance.
 
Specifically, we obtain labeled source data $\{x_i\} \sim \mu$, where each data point is associated with a label $v_i$, and target data $\{y_j\} \sim \nu$ with unknown labels. For simplicity, we use $X$ and $Y$ to denote the random vectors following distributions $\mu$ and $\nu$, respectively. The two distributions $\mu$ and $\nu$ can be coupled in a way that each paired samples of $(X,Y)$ from the coupled joint distribution are likely to have the same label. In order to identify such coupling information between source and target data, we propose a new OT-based domain adaptation method --- DASPOT (Domain Adaptation with SPOT) as follows.

%We aim to train a classifier on the source data that can be adapted to classify the target data. % Existing methods use optimal transport to find a mapping that can align the source $X$ and the target $Y$.
%Given labeled source data $(X,l) \sim \mu$ and unlabeled target data $Y \sim \nu$ sharing similar characteristics (e.g. same classes and same input size), one would like to train a classifier on source data and can be used for the target data. Using optimal transport to find a mapping which can align $X$ and $Y$ is a natural formulation. However, limited by the high computation cost, OT can hardly be applied to large and high dimensional datasets (e.g. image data). Here we demonstrate the ability of SPOT to tackle domain adaptation in large scale. 

Specifically, we jointly train an optimal transport plan and two classifiers for $X$ and $Y$ (denoted by $D_X$ and $D_Y$, respectively). Each classifier is a composition of two neural networks --- an embedding network and a decision network. For simplicity, we denote $D_X = D_{e, X} \circ D_{c, X}$, where $D_{e, X}$ denotes the embedding network, and $D_{c, X}$ denotes the decision network (respectively for $D_Y = D_{e, Y} \circ D_{c, Y}$). We expect the embedding networks to extract high level features of the source and target data, and then find an optimal transport plan to align $X$ and $Y$ based on these high level features using SPOT. Here we choose a ground cost \begin{align}\label{DA-cost}
c(x,y) = \norm{D_{e,X}(x)-D_{e,Y}(y)}^2.
\end{align}
Let $G$ denote the generator of SPOT. The Wasserstein distance of such an OT problem can be written as $\EE_Z\norm{D_{e,X}(G_X(Z))-D_{e,Y}(G_Y(Z))}^2$.%which encourages $X$ and $Y$ to be paired together if the Euclidean distance between their embeddings is small. 

%We decompose $D_X$ and $D_Y$ into two parts: the embedding network and the classification network. Then we have $D_X = D_{e, X} \circ D_{c, X}$ and $D_Y = D_{e, Y} \circ D_{c, Y}$ with $D_{e, X}, D_{e, Y}$ being the embedding networks and $D_{c, X}, D_{e, Y}$ being the classification networks. 

Meanwhile, we train $D_X$ by minimizing the empirical risk $\frac{1}{n}\sum_{i=1}^n[\cE(D_X(x_i),v_i)]$, where $\cE$ denotes the cross entropy loss function, and train $D_Y$ by minimizing 
\begin{align}\label{DA-risk}
\EE_Z[\cE(D_Y(G_Y(Z)),\argmax_{k}[D_X(G_X(Z))]_k)],
\end{align}
where $[v]_k$ denotes the $k$-th entry of the vector $v$. The risk function defined in \eqref{DA-risk} essentially encourages $D_X$ and $D_Y$ to predict each paired (synthetic) samples of $(G_X(Z),G_Y(Z))$ to have the same label.

Eventually, the joint training optimize 
\begin{align*}
\min_{D_X,D_Y,G}\max_{\lambda_X,\lambda_Y}\cL_c(G,\lambda_X,\lambda_Y) + \frac{\eta_{\textrm{s}} }{n}\sum_{i=1}^n[\cE(D_X(x_i),v_i)]
+ \eta_{\rm da}  \EE_Z[\cE(D_Y(G_Y(Z)),\argmax_{k}[D_X(G_X(Z))]_k)],
\end{align*} where $\cL_c(G,\lambda_X,\lambda_Y)$ is the objective function in \eqref{eq:finalvariant} with $c$ defined in \eqref{DA-cost}, and $\eta_{\rm s}, \eta_{\rm da}$ are the tuning parameters. 


==> conclusion.tex <==
%!TEX root = ./ICML2019_Paired_GAN.tex

\vspace{-0.15in}
\section{Conclusion}
\vspace{-0.1in}
We propose the SPOT (Scalable Pushforward of Optimal Transport) framework to efficiently solve optimal transport problems. Specifically, we approximate optimal transport plan as a generative model parameterized by a deep neural network, and cast the optimal transport problem into a minimax optimization problem. We then introduce how to recover the density of the transport plan. Numerical experiments illustrate that SPOT not only has favorable convergence behavior, but is also capable to efficiently generate authentic samples. We finally apply SPOT to domain adaptation problems and achieve state-of-the-art performances. 
